Balancing Efficiency and Empathy: Healthcare Providers' Perspectives on AI-Supported Workflows for Serious Illness Conversations in the Emergency Department

Serious Illness Conversations (SICs), discussions about values and care preferences for patients with life-threatening illness, rarely occur in Emergency Departments (EDs), despite evidence that early conversations improve care alignment and reduce unnecessary interventions. We interviewed 11 ED providers to identify challenges in SICs and opportunities for technology support, with a focus on AI. Our analysis revealed a four-stage SIC workflow (identification, preparation, conduction, documentation) and barriers at each stage, including fragmented patient information, limited time and space, lack of conversational guidance, and burdensome documentation. Providers expressed interest in AI systems for synthesizing information, supporting real-time conversations, and automating documentation, but emphasized concerns about preserving human connection and clinical autonomy. This tension highlights the need for technologies that enhance efficiency without undermining the interpersonal nature of SICs. We propose design guidelines for ambient and peripheral AI systems to support providers while preserving the essential humanity of these conversations.

==> sections/Related_work_7.28.tex <==
\section{Related Work}
% Outline:
% Briefly introduce the SI, SIC. 

% --
% Focus on what makes SIC in the emergency department different / unique, what is the characteristic of SIC in ED; (Busy, emergency, etc.). 
% ----- Current stage of the SIC in the real world: Briefly introduce SIC in ED with elder adults;  Not enough. Older Adults needs more;  


% Seconde paragraph: 
% - Patients and doctor communication?  --- why we need this.

% AI to support:  
% - Design of AI-based tools to support patient-provider communication? 
% - AI techniol;l
\subsection{Serious Illness Conversation With Older Adult Patients in Emergency Department}

Serious illness refers to ‘a health condition that carries a high risk of mortality and either negatively impacts a person’s daily function or quality of life, or excessively strains their caregivers’ ~\cite{kelley2018identifying}. According to a survey, three-quarters of adults aged 65 and older live with at least one serious illness\cite{statista2022serioushealth}. For this population, SICs enable patients to articulate their values, goals, and care preferences, allowing clinicians to develop treatment plans that align with their wishes~\cite{houben2014efficacy,silveira2010advance} and can reduce both the frequency and duration of unnecessary hospitalizations~\cite{klingler2016does}. However, many older adults have never participated in an SIC~\cite{prachanukool2022emergency}. Even among those who had SICs, their care preferences naturally evolve over time~\cite{kim2016natural}, creating persistent challenges in ensuring care aligns with evolving goals.

The Emergency Department (ED) represents a particularly critical setting for SICs~\cite{prachanukool2022emergency}. As the important entry point into the hospital system~\cite{ouchi2019goals}, EDs are where initial treatment plans are formulated. Older adults account for one-quarter of ED visits~\cite{galvin2017adverse}, with many arriving in life-threatening conditions - half are in their last month of life, and three-fourths are within six months of death~\cite{wilson2020end}. This population faces an average 10\% mortality rate and 24\% rate of ED revisits and readmissions\cite{aminzadeh2002older}. Timely SICs in this setting can reduce aggressive interventions, decrease surrogate stress, and improve alignment with patient values~\cite{ouchi2017preparing}.

Despite this critical need, SICs remain underutilized: fewer than one-third of older adults in EDs engage in such conversations~\cite{clark2018racial}. Clinicians face multiple barriers including severe time constraints (average ED stays of four hours~\cite{ouchi2019goals}), lack of structured protocols~\cite{ouchi2019goals}, and concerns about triggering negative emotional responses~\cite{shilling2024let}. 
Additionally, prognostic uncertainty often leads to clinician over-optimism~\cite{christakis2000extent}, which patients may internalize, resulting in preferences for overly aggressive care. 

Existing frameworks attempt to address these challenges. 
The Serious Illness Conversation Guide (SICG)~\cite{bernacki2015development} is a validated framework that offers a structured sequence of open-ended questions. The Serious Illness Care Program (SICP) adds training and workflow reminders~\cite{paladino2020training, paladino2023improving}. However, these tools are often not well-suited to the dynamic and time-pressured ED context. SICG takes more than 20 minutes to complete~\cite{mandel2023pilot} and the fixed questions are not adaptable to varying clinical scenarios. SICP does not fully alleviate the emotional burdens clinicians facing~\cite{paladino2023improving}. 

These limitations highlight the need for novel approaches tailored specifically to ED workflows. However, limited research has examined the specific workflow of conducting SICs in EDs or identified the unique needs and challenges clinicians face in this high-pressure environment. This gap in understanding ED-specific SIC workflows and requirements forms the foundation for our first research question.

\subsection{Technology-supported Patient-Provider Communications}

Effective patient-provider communication is fundamental to patient-centered care~\cite{sunnerhagen2013enhancing}, improving patient engagement~\cite{butz2007shared}, reinforcing positive expectations~\cite{wright2004doctors}, and enhancing mental health outcomes~\cite{wong2019associations}. 

The HCI community has increasingly recognized communication as a critical design space for healthcare technologies. Various technological interventions have been developed to support patient-provider communication~\cite{ryu2023you, ramesh2024data, seljelid2021digital}. Notable examples include BodyDiagrams, which enables patients to annotate pain intensity and timing on a body map~\cite{jang2014bodydiagrams}; recovery dashboards that facilitate joint data interpretation between stroke patients and clinicians~\cite{ramesh2024data}; and mobile applications that surface family-reported needs in ICUs to prompt palliative care consultations~\cite{cox2025mobile}. Additionally, researchers have developed communication feedback tools to help clinicians recognize and address implicit bias in real-time interactions~\cite{bascom2024designing}.

A subset of these technologies specifically targets the elicitation of patient values and care preferences~\cite{sudore2017effect, berry2021supporting}. For example, Living Voice~\cite{vitaldecisions_mylivingvoice} allows patients to document treatment wishes for sharing with family or providers, while Foong et al.~\cite{foong2024designing} proposed five value-elicitation tools focused on caregiver input. Curtis et al.~\cite{curtis2023intervention} introduced the Jumpstart Guide, which  automatically extracts EHR data to generate conversation templates for clinicians.

However, these tools are predominantly designed for low-pressure care settings where patients have time to reflect and clinicians can engage in unhurried conversations. The ED presents fundamentally different challenges: high-pressure situations, time constraints (typically four-hour stays~\cite{ouchi2019goals}), patients in crisis, and limited prior rapport.
Existing tools may not address the urgency, emotional intensity, or rapid decision-making demands characteristic of ED-based SICs with older adults.


\subsection{AI Technologies in Supporting Patient-Provider Communications and SICs}

Researchers have explored AI-powered Conversational Agents (CAs) to enhance patient-provider interaction. Yang et al. 
~\cite{yang2024talk2care} developed Talk2Care, an LLM-powered telehealth system that enables older adults to share health information through voice interfaces while providing clinicians with AI-generated conversation summaries. Similarly, Li et al.~\cite{li2024beyond} created a GPT-4 chatbot that streamlines pre-visit workflows by collecting patient information and generating interactive summaries for clinical teams. Hao et al.~\cite{hao2024advancing} built an interactive AI system that supports older adult cancer patients to collaborate with their cancer care clinicians during consultations. Seo et al.~\cite{seo2025enhancing} designed an AI chatbot to facilitate communication between pediatric patients, parents, and healthcare providers during clinical visits.


Given the complexity of SICs, researchers have explored various AI approaches to support clinicians. One line of work focuses on patient identification and workflow integration. For example, AI algorithms have been developed to predict patient mortality rates, helping clinicians efficiently identify high-risk patients who would benefit from SICs~\cite{avati2018improving}. Manz et al.~\cite{manz2020effect} demonstrated that combining AI mortality predictions with automated reminders increased SIC frequency among oncology clinicians.

Another research direction addresses SIC documentation and analysis. Natural language processing techniques have been developed to identify previous SIC documentation in EHRs to extract SIC content from clinical notes~\cite{lindvall2022natural}. Hachem et al.~\cite{hachem2025electronic} created dashboards to track clinician SIC training progress and facilitate conversation documentation.

Another line of research proposed an AI-human collaborative workflow for conducting the SIC~\cite{chua2022enhancing}.
Before the SIC, they suggested using CAs to collect the needed patients' information to better prepare for SICs.
After the SIC, they highlighted the potential of using NLP to improve both the efficiency and quality of SICs documentation.
Given AI's potential to evaluate communication skills in clinical settings~\cite{ryan2019using}, they also proposed leveraging AI to analyze previous SICs and provide feedback to healthcare providers.

\textbf{Research Gap and contribution}

While this body of work demonstrates AI's potential in healthcare communication, significant gaps remain in understanding how clinicians want AI support for SICs, particularly in high-stakes ED environments. Existing research has primarily focused on technical feasibility rather than user-centered design considerations. From an HCI perspective, it remains unclear what AI capabilities would be most valuable to ED clinicians, how such tools should integrate with existing workflows, and what design principles should guide AI-supported SIC tools for time-constrained, emotionally intense clinical encounters. 

This gap in understanding clinician needs and preferences for AI-supported SICs in ED settings forms the foundation for our second research question.









==> sections/draft__V2__interview_with_ten_healthcare_providers.tex <==


\section{Interviews with Healthcare Providers Working in the ED}
Based on the formative expert interviews, we identified four key steps in the healthcare provider's workflow for conducting SICs with older adults in the ED. 
In the subsequent semi-structured interviews, we engaged with a broader group of healthcare provider members to gain a deeper understanding of the specific challenges and needs they encounter at each step of this workflow, as well as their perspectives on how AI technologies might support their practices.


\subsection{Study Participants}
The participants in this study were healthcare providers who practice in the ED and have experience conducting SICs with older adults. While they do not specialize in or conduct research on serious illness communication, they routinely engage in these conversations as part of their clinical responsibilities. Their work environment is high-pressure and fast-paced, often involving complex cases and rotating day and night shifts, which makes their availability limited. 
To capture a holistic understanding of the interprofessional workflow and communication dynamics involved in SICs, we intentionally recruited nine U.S.-based healthcare providers across diverse roles, including two nurses and seven physicians.
Participants were identified through the professional networks of our expert interviewees and recruited using snowball sampling—a commonly used method for accessing highly specialized clinical populations.
Table~\ref{tab:demographics2} shows our participant demographics, department, roles, and years of practice.
%Our study was reviewed and approved by the first author's institution's Institutional Review Board, and the study complied with the approved procedure for ethical research practices of human subject protection.

\begin{table*}
  \caption{Demographics of the Subsequent Semi-Structured Interviews}
  \label{tab:demographics2}
  \begin{tabular}{cclcc} 
    \toprule
    P\# & Gender & Department & Job Title & Year of Practice \\ 
    \midrule
    P1 & Male & Emergency Department & Emergency Medicine Physician and Toxicologist & 30 years \\ 
    P2 & Female & Emergency Department & Nurse & 42 years \\
    P3 & Male & Emergency Department & Emergency Medicine Physician & 10 years \\ 
    P4 & Female & Emergency Department & Emergency Medicine Physician & 4 years \\
    P5 & Male & Emergency Department & Emergency Medicine Physician & 7 years \\ 
    P6 & Female & Emergency Department & Nurse & 20 years \\
    P7 & Male & Emergency Department & Emergency Medicine Physician and Intensivist & 20 years \\ 
    P8 & Male & Emergency Department & Emergency Medicine and Palliative Care Physician & 5 years \\
    P9 & Male & Emergency Department & Emergency and Critical Care Medicine Physician & 5 years \\
    \bottomrule
  \end{tabular}
\end{table*}

\subsection{Study Procedure}
We conducted semi-structured interviews remotely via Microsoft Teams, each lasting approximately 30 minutes.
Participants first described a recent experience conducting an SIC with an older adult in the ED. 
They then detailed specific challenges and needs experienced during each phase of their workflow (identification, preparation, conduction, and documentation).
Next, participants shared the existing frameworks and technologies they currently rely upon to support their SIC processes. 
Finally, we explored participants' perspectives regarding potential roles for AI technologies.

To support participants in reflecting on AI opportunities, we used insights from earlier expert interviews to create illustrative examples of text-based AI support.
These were not part of the interview protocol per se, but were used only if participants struggled to articulate scenarios on their own.
Our intention was not to test these scenarios or restrict the conversation but rather to use them as reflective scaffolds—cognitive prompts that could help participants generate or refine their own ideas. 
Participants were encouraged to respond freely, expanding upon, critiquing, reframing, or entirely redefining the scenarios provided.
This approach reflects early-stage, exploratory design research practices where speculative but grounded examples can support participants’ imagination while preserving openness and participant agency.
The interviews were audio-recorded and transcribed with the participants' consent. 



After the interviews, we analyzed transcripts using both inductive and deductive thematic analysis methods~\cite{fereday2006demonstrating}. 
Two researchers from our team independently employed the inductive thematic analysis approach to analyze two transcripts and identified meaningful quotes, and categorized these quotes into codes. 
Then, they resolved discrepancies among the codes and came up with key themes.
After the discussion, they used deductive thematic analysis to group similar codes and leveraged inductive thematic analysis to identify new codes.
They then discussed again and reached a consensus about the codes.
Finally, they grouped the codes into themes in each step of the SIC workflow.
To transparently report our findings, we indicate the prevalence of codes and themes across participants using the following terminology: "a few" refers to up to 20\% of participants, "some" indicates 21-50\%, "most" represents 51-80\%, and "nearly all" denotes 80\% or more of participants.







\section{Findings}
\label{sec:finding}
In this section, we presented the challenges and needs (Sections \ref{sec:identification} through \ref{sec:documentation}) that healthcare providers face in their workflow of conducting SICs with older adult patients in the ED to address RQ1. 
Then we discussed AI opportunities (Section \ref{sec:ai}) to address RQ2.
Key findings are summarized and visualized in Fig. \ref{fig:key_findings}.


\begin{figure*}[htbp]
  \includegraphics[draft=false,width=\textwidth]{Figures/key_findings.pdf}
  \caption{In this figure, we present the key challenges healthcare providers face at each stage of their workflow when conducting SICs. Moreover, we identified AI opportunities for addressing each of these challenges. Based on the findings, we developed four design guidelines, which we discuss in the discussion section. }
  \label{fig:key_findings}
   \Description{}
\end{figure*}



\subsection{Barriers to Identifying Which Patients Require SICs Due to Fragmented Documentation and Lack of Early Patient Identification}
\label{sec:identification}


In this section, we identified two factors that hinder SIC \textcolor{cyan}{\textbf{Identification}}: fragmented EHR documentation and a lack of early patient identification.
This extends beyond previous findings that focused primarily on prognostic uncertainty as the barrier to identification~\cite{shilling2024let}.

When older adult patients arrive at the ED with life-threatening conditions (e.g., brain bleeding) requiring aggressive treatment, healthcare providers enter the identification phase to determine whether SICs are necessary.
Healthcare providers typically begin this process by consulting the electronic health record (EHR) to locate documentation from previous SICs, which contains critical decision-making information, including code status (resuscitation and intubation preferences), care preferences, treatment goals, and patient values.
When this documentation is readily accessible, providers can make treatment decisions—whether to pursue aggressive intervention or comfort care—that align with the patient's established goals without initiating SICs.
However, when prior SIC documentation is unavailable or insufficient, providers have to conduct these conversations directly with patients to discuss treatment options and guide clinical decisions.
Unfortunately, many participants (P4, P5, P7, P8, P9) reported significant difficulties locating existing SIC documentation within the EHR sections designated for this information.
These challenges persist even when using keyword searches, which often yield incomplete results. 
For instance, when P8 searched for specific care preference terms, the EHR system returned "not addressed," which failed to provide the essential information needed to support informed clinical decision-making.

\begin{quote}
\textit{``If you open up a patient's chart on the left hand, most column where they're demographic information is if they've previously had, but it's really limited information that's captured [in a patient's chart]. So it's usually just like a DNR DNI status to not resuscitate, do not intubate......If patients have had more extensive goals of care discussion, it's not always easily accessible. Usually just the DNR DNA status. ''} (P4)
\end{quote}


The key factor underlying these accessibility challenges is inconsistent documentation practices for where to record SICs, which results in SIC-related information being scattered across multiple locations within patient records. 
As P9 explained, some healthcare providers document SICs by creating separate ED progress notes, others include information in ED final notes, and some use advance care planning (ACP) notes.
When SIC-related information is documented outside the standardized ACP note format, it becomes effectively invisible to other providers to locate this critical information.
The inconsistent documentation practices explain why healthcare providers frequently cannot access patients' previously documented code status, goals, and values precisely when this information is most needed for time-sensitive treatment decisions.

\begin{quote}
\textit{``I've seen variability where I've seen some people document it as a separate ED progress note. I've seen some people document as an ACP note. And then I've also seen some people just document it as part of the ED course that then populates into the final ED provider note.''} (P9)
\end{quote}



When healthcare providers cannot locate SIC documentation in the EHR, they resort to directly asking patients whether SICs have occurred previously.
However, many participants (P5, P6, P7, P8) discovered that many patients had never engaged in these critical discussions at all. 
This gap can stem from a systematic perspective where the medical system's lack of standardized protocols for proactively identifying patients who would benefit from SICs early in their illness trajectory, before acute crises develop.
Without early identification, SICs become reactive conversations triggered by emergencies rather than proactive discussions integrated throughout the patient's care journey.
Therefore, establishing early identification protocols is crucial not only for ensuring patients receive care aligned with their goals and values from the outset of their illness but also for equipping ED providers with the essential information needed to make rapid, patient-centered decisions during critical moments.


\begin{quote}
\textit{``I find a lot of oncologists do not have these discussions with patients about advanced care and we are having to do that (SIC) in real time with limited information in the emergency department....Our team would greatly appreciate that these discussions are made with family and the patient when they're alert and together and can think through the process...Victims of cancer and long-term disease have not had these conversations, or at least they're not documented in their chart, which makes it challenging for us in the ER to make these decisions.''} (P1)
\end{quote}



%Although some patients are available to talk, others are not. Some older adult patients arrive at the ED with acute deterioration and are unconscious, which makes it impossible to speak with them.
%Although patients are the preferred source for this information, speaking with surrogates or family members is also an option.
%However, family members are not always present when the patient arrives. 
%When neither the patient nor their family is available, providers are left with only one option: to proceed with aggressive treatments such as intubation in an effort to save the patient's life, despite the risk that these actions may not align with the patient's goals and values.

%\begin{quote}
%\textit{``And oftentimes you get older individuals who don't have family members, or they can't be identified, and it makes the treatment sometimes trickier because they can't tell the story.''} (P1)
%\end{quote}


Even in cases where providers successfully locate existing SIC documentation, additional challenges emerge regarding information currency and accuracy.
Several participants (P3, P7) reported encountering situations where patients' goals of care and treatment preferences had evolved over time without corresponding updates to their medical records. 
This temporal disconnect creates uncertainty about whether existing documentation truly reflects patients' wishes, which makes it difficult for providers to determine when SICs are needed.
As a result, a few participants (P3, P7) emphasized that access to accurate and up-to-date patient information is essential for effective clinical decision-making.

\begin{quote}
    \textit{``The information documented in the chart may not be accurate, the goals of care may have changed, and haven't been updated. Sometimes there's conflicting notes, and understanding what's right and current can be helpful.''} (P3)
\end{quote}






\subsection{Negative Personal Experiences and Poor Logistical Conditions Add Psychological Burden on Healthcare Providers During Preparation of SIC}
\label{sec:preparation}

When patients are identified as needing an SIC, healthcare providers move to the \textbf{\color{magenta}{preparation}} phase.
While professional training may equip healthcare providers to handle emotionally intense situations, our interviews revealed that personal experiences can significantly complicate the preparation, particularly in the ED (P1, P5).
For example, P5 described how his father's death from cancer left emotional trauma that now makes the preparation more difficult.
He found these conversations more emotionally charged and noted becoming visibly affected, tearing up during conversations where he previously maintained composure. 
This finding reveals that even highly trained healthcare providers are not immune to the psychological effects of personal experience when preparing for SICs, particularly when the patient's condition mirrors that of the loved one they lost.


%For example, P1 described how caring for his parents during their end-of-life period gave him greater empathy and confidence when approaching SICs.
%He explained that going through the process of respecting his parents’ wishes, ensuring their comfort, and ultimately letting them go—despite the emotional difficulty—helped him understand the kinds of emotional challenges that families often face when making similar decisions.

%\begin{quote}
%\textit{``Also, having gone through long-term care with my parents have helped because personally I realize what it's like to have a parent and respect their wishes and make them comfortable and have to let them go because that's what they wish. Sometimes it's very hard for family members to make that decision, and often times they don't want that family member to be gone even if the family member wishes that. Their life be ended. So I've been through it.''} (P1)
%\end{quote}




\begin{quote}
\textit{``And then even the, the provider, the clinician comes with a lot of their own baggage. So, for example, you know my father passed away in 2021 from COVID. That next year or two, I was emotionally different than I was before. These conversations were more emotional for me. I was more connected to the conversation as I just lost my father. Even I might tear up during these conversations when historically throughout my career, I never would cry or show emotion like that.''} (P5)
\end{quote}


Beyond personal experience, logistical constraints (time and space) further compound the psychological burden of the preparation of SICs.
First, some participants (P4, P7, P8, P9) described challenges in finding an available time slot.
The high patient volume in the ED forces healthcare providers to manage multiple cases simultaneously, creating constant interruptions and time pressure.
Therefore, this environment increases cognitive load and emotional strain during preparation, particularly when SICs require emotional presence, careful communication, and active listening.

Moreover, space limitations create additional preparation challenges.
Some participants (P3, P4, P6, P8, P9) noted that having access to a private and quiet room is important not only for helping patients and their family members remain calm, but also for supporting healthcare providers emotionally in conducting emotionally charged SICs.
However, the ED's overcrowded and chaotic environment makes such spaces scarce (P8).
For example, some patients wait 10-15 hours in crowded rooms, and some are placed in noisy hallways, which leaves virtually no private spaces available for sensitive conversations.
Together, insufficient time and inadequate space intensify healthcare providers' psychological burden to prepare SICs and thus make SICs hard to conduct.

These preparation challenges, combined with personal trauma, create multiple barriers that cause healthcare providers to hesitate when initiating SICs. 
This extends beyond previous research that attributed such hesitation primarily to training deficits~\cite{ouchi2019goals} and concerns about causing emotional harm to patients~\cite{shilling2024let}, as discussed in our introduction.
Our findings emphasized healthcare providers' emotional needs, rather than focusing solely on patients' emotional needs when preparing for SICs.


\begin{quote}
\textit{``I think in the emergency setting, it is usually [challenging] like physical, like [finding] time and space [to conduct SICs]. So like I said, you know, even finding private care space sometimes is challenging. Having the time to have these conversations is really challenging.''} (P4)
\end{quote}






\subsection{Need for Patient-Specific Information and Contextualized Guideline to Support SICs Conduction in Emergency Care}
\label{sec:conduction}


Preparation for SICs is already challenging; however, these challenges can intensify during the \textbf{\color{brown}{conduction}}, particularly when initiating and progressing through SICs.
Many patients are cognitively overwhelmed, emotionally unprepared, and, in some cases, unreceptive to discussing their care preferences and deciding between “live” (aggressive treatment, but can cause irreversible damage) or “die” (reduce their pain but not prolong their lives) in a short period. 
On the other hand, both the nurse (P2) and the physician (P9) mentioned that family members often hold unrealistic hopes that the patient will return to full health, which leads these family members to engage in SICs to talk about the “crucial reality” of the possibility of losing their loved ones. 
These emotionally charged dynamics complicate SIC delivery while intensifying psychological burden on providers, particularly those already struggling with preparation.
As a result, healthcare providers' capacity to manage and respond to others' emotional distress becomes compromised, which creates a downward spiral that hinders effective SICs in the ED.


\begin{quote}
\textit{``You know you're talking to a family member of a young child, very difficult conversation, very difficult. The moment you add a child into the, the as the patient, it it becomes, it's hard to have these conversations. The more sudden and unexpected the emergency is, the more difficult the conversation is. The family or the patient, they're just not prepared. You know, like to tell a, a family member that, you know, that their 50-year-old husband who was just mowing the lawn and playing soccer with their son, now just had a massive heart attack...It's a different conversation.''} (P5)
\end{quote}

The primary reason for this challenge is that patients often lack a clear understanding of their current medical condition or the potential poor prognosis of their illness. 
This reflects a gap in patient-provider communication prior to their arrival at the ED, where few, if any, discussions about the progression of their illness have taken place.
To deal with the challenge, some participants (P2, P5, P6, P9) emphasized the importance of building a personal connection with the patient. 
They believed that having a connection with patients makes conversation more personal. 
As a result, patients may be more open to receiving difficult information and more willing to engage in the discussion.
P2 suggested breaking the ice by finding shared interests, such as sports teams or children.


However, some participants (P2, P5, P8) still face challenges in building the connection.
For example, P5 noted that, unlike in primary care, where providers have time to get to know patients and build connections, providers in the ED often meet patients for the first time under urgent and stressful conditions. 
Therefore, it becomes much harder for healthcare providers to build a connection with patients in the ED.
To address this challenge, supplying patient-context information (e.g., family support, personal interests such as favorite sports teams) before SICs is essential, which helps providers quickly understand patients and build personalized strategies to conduct SICs.

\begin{quote}
\textit{``We're at a significant disadvantage in the emergency department as I am not their primary care doctor. I have not cared for them for a decade, you know, and earned all their trust and faith. They are meeting me at point blank, you know, and they have to develop faith and trust.''} (P5)
\end{quote}




Although SICG is available to support in conducting SICs, they are primarily designed for clinical settings where the patient’s condition is stable and there is enough time and cognitive capacity, on both the provider and patient sides, to engage in reflective SICs.
Current guidelines and training fall short in supporting healthcare providers in conducting SICs in the ED context.
First, current guidelines and training do not offer practical ways to personalize icebreakers that could help providers initiate SICs with patients they first meet.
Moreover, there is little guidance on how to communicate a poor prognosis in a way that minimizes additional cognitive and emotional strain on patients and their family members.
Third, there is no clear support for helping providers de-escalate heightened emotions and move the conversation forward in a limited timeframe. 
These limitations point to the need for providing patient-specific information and contextualized support that are specifically designed for a time-constrained and high-pressure ED.


%To deal with this situation, healthcare providers (P8, P9) have to narrow the scope of the SIC and ask a few key questions that can support urgent clinical decision-making.

%\begin{quote}
%\textit{``......with a trusted oncologist or a primary care Doctor Who knows the patient really well. And that might address a lot of other things more globally around what's important to you in life and with your overall health. And for us in the ER, it's usually much more focused on the specifics or of do we do this thing or not, based on what your loved one would want and where they are in their health or illness. But I think it can be done pretty well in just a couple of minutes.''} (P8)
%\end{quote}


%\begin{quote}
%\textit{``I think it's often challenging when the goals of care don't necessarily align with reality. And there's an expectation that the patient's gonna recover from a condition that's essentially not recoverable. Or the expectations of the family or that there's going to be some type of sort of miraculous cure when that's not going to happen, that can be challenging.''} (P3)
%\end{quote}





\subsection{Lack of Systematic Protocol Hinders Effective SIC Documentation}

\label{sec:documentation}

When healthcare providers successfully overcome the numerous challenges of conducting SICs, they enter the \textbf{\color{teal}{documentation}} phase, where they must summarize each conversation as a note in the EHR system.
However, this phase presents its own significant obstacles.
As participants (P5, P8) described, the documentation process is a time-consuming and burdensome task, particularly for healthcare providers working in the ED. 
Given the high workload in the ED, providers have limited or no time for documentation during their scheduled shifts.  
Consequently, many providers must stay late or use unpaid personal time to complete this task; time that could otherwise be spent caring for additional patients.
Moreover, the challenge is compounded by the absence of effective documentation methods. 
As P8 noted, no standardized approach exists for documenting SICs, further complicating an already difficult process.

\begin{quote}
\textit{``A lot of what you do is looking through a ton of data, trying to synthesize it, seeing the patient, addressing too many things in too little time, and then trying to document it and then do it, you know, 30 or 40 more times in a shift. And so many of us end up staying late or working unpaid hours, finishing charts because we care, and the system takes advantage of us.''} (P8)
\end{quote}

When we examined why the documentation is time-consuming and burdensome, we identified two primary factors: inadequate training and absence of standardized protocols.
First, training related to SICs focuses primarily on how to conduct the conversations themselves, but overlooks a crucial step in completing the SIC workflow—documentation.
Moreover, there is no standardized protocol for documenting SICs across different care provider teams.
The absence of systematic protocols leads to two key problems: 1) inconsistent practices where providers struggle to determine what information to extract from conversations and how to organize it within the EHR, and 2) varying documentation approaches where different providers record SICs using different structures and store them in disparate EHR locations.
Consequently, other providers struggle to locate and utilize previously documented patient goals and values, undermining their ability to make clinical decisions aligned with patient preferences (as we discussed in Section \ref{sec:identification}).
As a result, there is a need for a systematic protocol for documenting SICs in order to reduce the documentation burden and enhance the overall efficiency of the SIC workflow cycle.





Although documentation represents the final step in the SIC workflow (individual level), P8 and P9 emphasized that it also serves as the starting point and foundation for subsequent SICs with other healthcare providers (organizational level).
As noted in Section \ref{sec:identification}, many older adult patients arriving in the ED have neither previously participated in nor documented SICs. Consequently, SICs conducted in the ED often generate a patient's first SIC documentation. 
However, due to severe time constraints in the ED, healthcare providers typically have only about 10 minutes to elicit patients' care preferences and make urgent treatment decisions, rather than the 50 minutes needed to explore broader values and goals comprehensively.
This initial documentation, therefore, becomes essential but incomplete groundwork that requires future, more comprehensive SICs as patients move through the healthcare system.




\begin{quote}
\textit{``And so really having a clear sense as you go into the conversation about what your goal is, I think that can be challenging because ultimately I think in the arc of a patient's illness, we might have the goal of of really getting clear understanding of their functional status of their preferences and then making a recommendation. But often times doing all of that, that conversation, if you have it all at once, can easily be a 45 minute to 90 minute conversation. And that is not available in the emergency department. And so you have to basically decide I can't do all of that.''} (P9)
\end{quote}

To complete the broader spectrum of SICs, collaborative efforts across multiple healthcare providers are required to build up a holistic picture of patient values, goals, and care preferences. 
However, the current EHR system has limited support for this collaborative effort.
One example is that when P1 wanted to find other providers to discuss patient treatment plans, the EHR system displays the contact information for multiple clinical care team members (e.g., attending physicians, residents, nurse practitioners), which makes it unclear whom he should contact.


\begin{quote}
\textit{``You'll open up a patient's chart and there'll be so many healthcare providers, physicians, nurse practitioners, physician assistants, residents...You don't know who to call, and if you do, they're often not on calls.''} (P1)
\end{quote}

As a result, patients may experience inconsistent, misaligned care, as each point of care and SIC conducted across different departments remains disconnected.
Therefore, a systematic protocol not only needs to support documentation but also be able to support patient information sharing and communication between different departments.










\subsection{Integrating the AI System into the SIC workflow in the ED}
\label{sec:ai}


\subsubsection{Opportunities for Integrating the AI system into the SIC workflow in the ED}
\label{sec:opportunities_for_ai}

When asked about the potential role of AI technologies in their workflow, participants expressed strong interest in three areas that directly reflect earlier challenges: (1) AI-assisted summarization for identification and preparation, (2) ambient AI systems for real-time contextual and personalized support during SICs, and (3) AI-generated SIC notes for documentation.

First, building on the EHR access challenges identified in Section \ref{sec:identification}, some participants (P3, P4, P7, P8) suggested that the AI system could extract and summarize key information (e.g., previous SICs) from extensive health records to help healthcare providers quickly understand patient health conditions and patients' care preferences.
Consequently, healthcare providers could more efficiently determine whether a SIC is needed and subsequently develop personalized conversation strategies tailored to each patient's specific medical conditions during the preparation phase.

\begin{quote}
\textit{``Anyone who's previously documented, like if there was a goal of care button, I could click and it would go through everything that's been documented on a patient's chart. Because maybe they had a conversation with a social worker a few weeks ago or their primary care doctor, and I just don't have the time to click through every note.''} (P4)
\end{quote}


Moreover, addressing the psychological challenges that complicate SIC delivery (identified in Section \ref{sec:conduction}), some participants (P4, P5, P6) proposed ambient AI systems.
The ambient AI systems can passively listen to conversations (with patient consent) and generate real-time, contextual question suggestions. These AI-generated prompts would be dynamically tailored to the ongoing dialogue, supporting healthcare providers in maintaining meaningful conversations while alleviating psychological stress.
P6 explained that the AI-generated suggestions could be helpful for healthcare providers with less experience to conduct SICs. 




Finally, many participants (P1, P3, P4, P5, P7, P8) expressed a strong interest in AI-generated SIC notes to address the substantial documentation.
Because SICs can be lengthy, healthcare providers must distill large amounts of information into concise, clinically useful records. Therefore, it can be beneficial to use the AI system to extract key information from SICs and generate notes for healthcare providers to further document. Although AI-generated SIC notes can be useful, participants have different preferences for how this information is presented to them. 
For example, P3 suggested that the AI system could filter out unrelated conversation details and highlight patient goals and care preferences. In contrast, P9 prefers viewing the full conversation text with key information highlighted, while P1 wanted structured templates based on the SICs or word prompts to guide note creation.
Regardless of how the AI system is used to support documentation, P8 estimated that automating 80\% of documentation work with the AI system could cut post-shift charting time in half, freeing up time for direct patient care.
\begin{quote}
\textit{``But if AI could offload even say 80 percent of that (documentation) and then the other 20 percent you're tweaking and verifying the transcript or, you know, the output, that would save close to half of my working hours that I could actually be spending with seeing more patients.''} (P8)
\end{quote}







\subsubsection{Concerns About Integrating AI into the SIC workflow in the ED}
\label{sec:concerns_about_ai}

While participants expressed enthusiasm for AI support opportunities, they also articulated important concerns.
Their worries focused on three key areas: (1) human connection, (2) trustworthiness, and (3) clinical accuracy.


First, some participants (P1, P3, P5, P6, P9) concerned that the AI system might diminish the deeply human aspect of SICs. 
The interaction between patients and providers during SICs represents more than structured information exchanges; they are highly personal moments characterized by emotional depth. 
Consequently, introducing the AI system could lead healthcare providers to rely on technology-driven prompts during SICs, potentially reducing the genuine emotional engagement and connection that patients value.
For instance, P3 was concerned that patients could perceive AI-assisted conversations as mechanical rather than sincere, thereby undermining the quality of the interaction.
Moreover, some participants (P1, P4, P5, P6, P9) worried that AI integration might create distracting and disrespectful interactions when they attempt to build connections with patients. 
They emphasized that frequent or noticeable interaction with computer screens could disrespect the gravity and intimacy of these sensitive SICs.

\begin{quote}
\textit{``if there's a perception that the physician is just using an electronic tool to ask [the] right questions, that's not really sort of coming from the heart, that could be negatively perceived.''} (P3)
\end{quote}


Trustworthiness emerged as another critical concern. 
Some participants (P1, P5, P7) emphasized the necessity of thorough data validation before integrating AI into their workflows.
Specifically, P1 noted that personal adoption of the AI system would heavily depend on endorsements by trusted colleagues and credible evidence supporting AI's clinical validity.
Beyond trust between healthcare providers and AI systems, participants also highlighted the importance of maintaining patient trust. 
They emphasized that obtaining explicit patient consent and providing clear opt-out options to protect patient privacy is essential to preserve this trust.


Finally, some participants (P3, P4, P7, P9) expressed concerns about the accuracy and clinical relevance of AI summarization for documentation. 
They worried that the AI system might fail to adequately highlight information that is clinical important to healthcare providers.
For example, P4 was concerned that the AI system might elevate patient reports (e.g., chest pain) that are not important based on patients' unique conditions to clinically significant events.
If the AI system highlights these minor mentions, it could lead to unnecessary medical interventions and resource usage.
Such errors could result from the lack of clinical context or nuanced interpretation, further highlighting the importance of human oversight.
Thus, some participants (P3, P7, P9) emphasized the critical importance of clinician review and verification processes before finalizing any AI-generated summaries, ensuring their accuracy.

\begin{quote}
\textit{``Although the final sign off is going to be clinician reviewing the summary of what AI note taking would be, right?...We still have to read it again, make sure that's actually all accurate.''} (P7)
\end{quote}




==> sections/draft_initial_expert_interviews.tex <==
\section{Formative Expert Interviews}
To address RQ1 and RQ2, we began with formative interviews with two emergency physicians who specialize in SICs in the ED and conduct research at the intersection of emergency medicine and palliative care. 
These expert interviews served multiple critical purposes in our research design. 
Given that workflows of SICs in EDs are not standardized and often vary across institutions and among individual clinicians~\cite{paladino2021implementing, chua2022enhancing}, we first needed to understand the range of practices, adaptations, and challenges that arise in real-world contexts. 
The complexity and ethical sensitivity inherent in SICs required expert input to identify clinical norms, typical points of breakdown, and potential areas where AI technologies could offer meaningful support. 
These interviews helped us outline key moments and decision points that guided the rest of our study. 
Additionally, the expert interviews informed the development of our semi-structured interview guide for interviews with nine healthcare providers, which ensures the semi-structured interview guide was grounded in domain-appropriate language and clinical logic. 
This methodological approach helped us to examine how healthcare providers currently conduct SICs in practice, what challenges they face, and where they see opportunities for AI to enhance their workflows while maintaining clinical authenticity and relevance.



\subsection{Study Participants}

We recruited two highly experienced clinical experts (hereafter referred to as EX1 and EX2) through the professional networks of domain experts on our research team using convenience sampling~\cite{sedgwick2013convenience}.
\textbf{Both experts have substantial experience conducting SICs with older adult patients in the ED.}
They possess deep knowledge of the broader healthcare provider's workflow for conducting SICs and are familiar with the potential and limitations of AI technologies in clinical contexts.


EX1 is an emergency physician and home hospital physician as well as a nationally recognized clinical researcher. He serves as a clinical standard-setter for SICs in emergency medicine. In addition, he specializes in palliative care interventions for older adults with serious illness and leads a network of 400 emergency physicians focused on geriatrics and palliative care.
EX2 is an emergency physician and researcher working on developing AI-driven, automatable screening tools to identify older adults in the ED at high risk of six-month mortality. His research focuses on leveraging EHR data and automation to improve screening, SICs, and care delivery for older adults, particularly those with dementia or near the end of life.

Table~\ref{tab:demographics} summarizes expert demographics, departmental affiliations, roles, and years of clinical practice.
This study was reviewed and approved by the Institutional Review Board at the first author’s institution and conducted in accordance with ethical guidelines for human subjects research.


\begin{table*}
  \caption{Demographics of the Experts in Initial Expert Interviews}
  \label{tab:demographics}
  \begin{tabular}{cclcc} 
    \toprule
    Expert\# & Gender & Department & Job Title & Year of Practice \\ 
    \midrule
    EX1 & Male & Emergency Department & Emergency Medicine Physician & 7 years \\ 
    EX2 & Male & Emergency Department & Emergency Medicine Physician & 11 years \\
    \bottomrule
  \end{tabular}
\end{table*}



\subsection{Study Procedure}


We conducted two semi-structured interviews via Microsoft Teams, each lasting approximately 60 minutes. At the start of each session, the experts were invited to describe a recent experience conducting a SIC with an older adult in the emergency department. We asked follow-up questions about how they elicited patients’ goals and values, how those informed treatment decisions, how they collaborated with other care team members, and what tools or documentation practices they currently use.

Next, the experts walked us through the typical steps of their SICn workflow, highlighting key decision points and communication challenges. We then explored their perspectives on how AI technologies might support these workflows, including features they would find valuable and concerns related to trust, reliability, and integration into clinical practice.
Insights from these interviews were synthesized into a set of text-based probes that illustrated AI support opportunities (e.g., surfacing patient values, suggesting next conversational steps). These probes were later used in subsequent interviews with members of healthcare providers in EDs to prompt reflection and concrete feedback on potential AI functionality. This approach aligns with design research practices that prioritize participant-driven input while offering light scaffolding when exploring emerging technologies.

Experts were asked not to disclose any personally identifiable information during the interviews. With their consent, interviews were audio-recorded and transcribed. We conducted thematic analysis~\cite{braun2021thematic, braun2012thematic} to derive key themes, focusing on: (1) the overall workflow for conducting SICs in the emergency setting, and (2) expert perspectives on how AI technology could support this work.
Two members of the research team independently coded the transcripts to identify meaningful segments. Codes were iteratively grouped into themes, and discrepancies were resolved through collaborative discussion to finalize a consensus set of findings.

\begin{figure*}[htbp]
  \includegraphics[draft=false,width=\textwidth]{Figures/method_diagram.pdf}
  \caption{In this paper, we conducted a two-stage study. First, we carried out semi-structured interviews with two SIC experts to derive a four-step workflow for conducting the SICs in the ED. We also developed a set of text-based AI probes, which were subsequently used in interviews with nine healthcare providers. Based on the interviews with the healthcare providers, we addressed RQ1 and RQ2 by identifying the key needs and challenges in the SICs process, as well as AI opportunities and concerns. Finally, we derived design guidelines grounded in our findings.}
  \label{fig:two_stage}
   \Description{}
\end{figure*}



\subsection{Findings}

\subsubsection{Four-Stage Workflow of Conducting SICs With Older Adults in EDs}

Through our expert interviews, we identified four core phases in the workflow of conducting SICs with older adults in the ED: \textcolor{cyan}{\textbf{Identification}}, \textbf{\color{magenta}{Preparation}}, \textbf{\color{brown}{Conduction}}, and \textbf{\color{teal}{Documentation}}. 
In the ED, SICs are typically led by physicians, and occasionally by nurses. Depending on staffing and patient needs, social workers, physician assistants, and lay care workers may also contribute. Throughout the process, patients, their surrogates, and family members remain central participants.

During the \textcolor{cyan}{\textbf{Identification}} phase, healthcare providers determine whether they need to conduct a SIC with an older adult patient by recognizing two clinical indicators. 
The first involves direct clinical observation, including the patient's presentation, triage assessment, functional status, and acute condition.
If providers identify clinical decline, instability, or signs that a patient may be nearing end-of-life factors, this becomes a trigger for considering the need for SICs.
%talk about how these factors influence the decision about whether they want to have SICs with patients or not. (if they mentioned)
The second source is key information from the Electronic Health Record (EHR), particularly past visit history, treatment notes, code status\footnote{Code status refers to the level of medical intervention a patient wants in the event of a cardiac or respiratory arrest.}, and previously expressed values and goals.
Such EHR data serve as practical heuristics to help providers understand the patient’s longitudinal trajectory and treatment history. When providers observe the missing information,  or mismatch, such as a palliative intent with a full code \footnote{Full resuscitation – all resuscitative and aggressive curative treatment are provided. } order, or repeated ED visits without improvement, they may initiate a SIC to ensure goal-concordant care.
%maybe talk about why code status, and previously expressed values and goals are important in the identification phase.
For example, EX2 identifies patients who need a SIC through patterns of repeated ED visits and observable signs of decline.
EX1 flags cases where the treatment intent appears palliative but the patient remains listed as full code (e.g., intubate and resuscitate). Additionally, physiological decline or inconsistencies between a patient’s current condition and documented code status (e.g., Do Not Resuscitate (DNR) \footnote{Do Not Attempt Resuscitation (DNAR) or Do Not Resuscitate (DNR) – order designating that in the event of a cardiac or respiratory ARREST, resuscitation will not be attempted. All other aggressive treatment desired will be provided as appropriate. }/Do Not Intubate (DNI)\footnote{A DNI or “Do Not Intubate” order means that chest compressions and cardiac drugs may be used, but no breathing tube will be placed.}) often signal the need for SIC.
When these sources collectively suggest that the current care plan may not reflect the patient's goals and values, the team proceeds with initiating a SIC.

Once a patient is identified, the team moves into the \textbf{\color{magenta}{Preparation}} phase.
Although often brief in the ED, this phase lays the foundation for a productive conversation.
There are two parts in this stage: logistical planning and mental readiness. 
Logistical planning is to decide when and where the conversation should take place and who should be present. 
Mental readiness refers to clinicians who need to prepare themselves emotionally and cognitively to engage in what are often sensitive, complex discussions.  
This dual preparation helps ensure that healthcare providers can navigate the complex terrain of an SIC with appropriate sensitivity and clinical grounding.

The healthcare providers then enter the \textbf{\color{brown}{Conduction}} phase of the conversation, which represents the core interaction where values and goals are explored. 
This phase typically begins with an opening question to the patient or family that introduces the topic and initiates the dialogue in a sensitive manner. 
The care team first assesses what the patient and family understand about the current health condition and treatment, addressing any confusion or misinformation. 
The conversation then shifts to the heart of SICs: exploring the patient's goals, values, and any care trade-offs they find acceptable.
The conversation is adjusted dynamically, based on the patient's or family's stated preferences and priorities. 
The overarching aim of this phase is to reach a shared understanding of both medical realities and personal priorities both medical realities and patient priorities.
As a result, healthcare providers propose a plan of care that authentically aligns with what the patient values most.

Following SICs, the healthcare providers enter the \textbf{\color{teal}{Documentation}} phase.
Here, they record the outcomes of the SIC in the EHR, including the patient's goals, values, and care preferences.
This documentation serves as a reference for other clinicians, supports continuity across care transitions, and provides a lasting record to guide future decisions. 
Beyond formal documentation, the teams also encourage patients to follow up with specific providers about their condition or care plan. 
High-quality, accessible documentation is essential to ensure that multiple clinical teams beyond the ED can deliver continuous, goal-oriented care.
We summarize SICs' workflow in Fig. \ref{fig:workflow_ui}.

\begin{figure*}[htbp]
  \includegraphics[draft=false,width=\textwidth]{Figures/workflow.pdf}
  \caption{Four phases in the healthcare provider’s workflow for conducting SICs with older adult patients in the ED: (1) Identify the older adult patients, (2) prepare for SICs with the patients mentally and logistically, (3) conduct SICs, (4) document the key information from SICs.}
  \label{fig:workflow_ui}
   \Description{}
\end{figure*}

\subsubsection{AI Opportunities in Supporting the Healthcare Providers' Workflow}
After two experts talked about the workflow of conducting SICs, they showed a high interest in integrating AI into their workflow. 
Two areas emerged as promising: generating conversation guidance during SICs and receiving feedback to improve communication skills.
During the conduction phase, EX2 explained that although clinicians have access to existing guidelines with recommended questions, the number of options can be overwhelming in real-time, especially under ED time constraints.
Both experts shared that an AI system capable of listening to the conversation, while preserving privacy and consent, and offering real-time, context-aware suggestions for follow-up questions could be beneficial.
In addition to in-the-moment support, EX2 highlighted the lack of feedback following SICs.
Without insight into what questions were missing or how questions could be better framed, it is difficult to improve the SIC skills over time.
Thus, EX2 noted that an AI tool capable of analyzing previous conversations and providing constructive, case-specific feedback could support ongoing learning.



==> sections/draft_introduction.tex <==


\section{Old Version -  Introduction}
%Serious illness conversation (SIC) is a form of care provider-patient communication, typically occurring in clinical settings with patients who are experiencing serious illness~\cite{ouchi2019goals} (e.g.,  cancer, cardiovascular disease~\cite{hamidpour2014summer}). 
%Through SIC, clinical care teams elicit patients’ values (i.e., fundamental beliefs about life and self, such as the will to be alive for one’s grandchildren~\cite{naik2016health}), treatment goals (e.g., curing the disease or on providing comfort), and care preferences (e.g., specific treatment)~\cite{shilling2024let}.
%By doing so, subsequent clinical decisions can align with patients’ values and preferences, which ensures care remains patient-centered.
%what they consider most important in life~\cite{friedman2013value}
%which leads to a patient-centered and goal-concordant care~\cite{geerse2019qualitative}.
%SIC is particularly important in the Emergency Department (ED).
%Patients in the ED normally arrive at an inflection point in their illness trajectory, and the urgent decisions (i.e., ICU admission or hospice referral) made by clinical care teams can shape the nature of patients' subsequent care. 
%the intensity of care determined in the ED often continues during the hospitalization~\cite{ouchi2019goals}
%Under this intense time pressure, SIC need to be conducted to help patients formulate their values and care goals and ensure that subsequent treatment aligns with their preferences.
%As a result, SIC helps ensure that the care patients receive aligns with their individual preferences~\cite{paladino2023improving, hachem2025electronic}, ultimately enhancing patients' satisfaction with the care~\cite{ouchi2017preparing} as well as the quality of their end-of-life experience~\cite{geerse2019qualitative}.



When patients live with serious illnesses such as cancer or cardiovascular disease, the conversations they hold with clinical care teams (e.g, physicians or nurses) become critically important~\cite{ouchi2019goals, hamidpour2014summer}. 
These serious illness conversations (SICs) make clinical care teams understand what matters most to patients during treatment. 
Specifically, SICs help patients clarify their fundamental values (e.g., the desire to be alive for grandchildren's milestones~\cite{naik2016health}), their treatment goals (e.g., pursuing curative treatment versus focusing on comfort care), and their specific care preferences (e.g., whether to proceed with intubation, placing a tube into the airway, or not)~\cite{shilling2024let}. Rather than simply discussing medical options, well-conducted SICs help patients feel heard, strengthen the therapeutic alliance, and ultimately create a foundation for patient-centered care that reflects patients’ own priorities.



The stakes of SICs become particularly acute in Emergency Department (ED) settings.
Patients often come to the ED during a pivotal stage in their illness trajectory~\cite{ouchi2019goals},
and urgent clinical decisions (e.g., ICU admission or hospice referral) must be made quickly.
Yet these decisions may fundamentally shape the entire trajectory of a patient's subsequent care. 
Because of the urgency and importance, a timely and well-conducted SIC is essential in the ED to help the care they receive align with patients’ values, treatment goals, and care preferences~\cite{paladino2023improving, hachem2025electronic}.
As a result, patients can have higher satisfaction with their care~\cite{ouchi2017preparing}, and optimized quality of their end-of-life experiences~\cite{geerse2019qualitative}.

%%
 

Older adults aged 65 and above represent the largest group needing SIC, yet are least likely to receive them \cite{wilson2020end}. 
These patients account for up to one-quarter of all ED visits in the U.S., totaling 156 million visits annually \cite{samaras2010older, pines2013national}. %yet often arrive with care needs that differ significantly from those of younger patients \cite{aminzadeh2002older}. 
Among these older adults, three-fourths of these patients would die within six months ~\cite{wilson2020end}, which makes the ED visit a critical moment to understand their goals and values for delivering goal-concordant end-of-life care. 
Despite this pressing need, up to 99\% of older adults in the ED lack documented treatment goals and care preferences ~\cite{ouchi2017preparing}. In the absence of such information, clinical care teams often default to aggressive interventions (e.g., chemotherapy, ventilation, or intubation 
 ~\cite{wright2008associations}) that some older adults describe as “worse than dying”\cite{Rubin_Buehler_Halpern_2016}.
 For instance, older adult patients who prefer comfort can receive intubation in the ICU, which can cause distressing sensations of suffocation ~\cite{knudsen2015awake}.
 %and both physical and psychological distress during an already challenging time~\cite{wright2008associations}.
 Additionally, patients without documented treatment goals and care preferences experience higher rates of anxiety and depression ~\cite{detering2010impact}, while receiving treatments that cost nearly double those of less aggressive approaches~\cite{teno2002medical}. 
Thus, conducting SICs to close this gap in the ED is an urgent need.


%Despite the importance of SIC, clinical care teams face significant challenges in conducting SIC and therefore rarely conduct SICs with older adult patients in the ED~\cite{ouchi2019goals}.
%\citet{prachanukool2022emergency} %studied 332 older adult patients and found that 63\% of the patients did not experience SIC in the ED.
%One major challenge they face is time constraints~\cite{adeyemi2024emergency}.
%Since the number of patients admitted to the ED can be up to 120 per day~\cite{jones2008forecasting},
%but there are only 25 beds available for patients~\cite{jones2008forecasting}, 
%it limits clinical care team capacity to conduct SIC with each patient with serious illness.
%In addition, clinical care teams are often unsure how to initiate SIC in the ED~\cite{ouchi2019goals}, which can reduce the chance of conducting SIC.
%In addition, clinical care teams feel unprepared for this conversation~\cite{chua2022enhancing} and emotional discomfort while addressing patients' emotional responses~\cite{geerse2019qualitative}, which can reduce their confidence to conduct SIC.
%Moreover, clinical care teams are often uncertain about patients' prognosis, and tend to be optimistic about patient conditions~\cite{christakis2000extent}, which can delay the initiation of SIC and hinder timely and accurate intervention.
%Moreover, clinical care teams often have inadequate training to conduct SIC~\cite{ouchi2017preparing, shilling2024let}, with only 29\% having received formal training ~\cite{fulmer2018physicians}.
%~\citet{fulmer2018physicians} studied 736 physicians and found that only 29\% had received formal training in SIC. 
%To support clinical care teams in conducting SIC, some frameworks and interventions have been implemented, such as the Serious Illness Conversation Guide (SICG)~\cite{bernacki2015development} and the Jumpstart Guide~\cite{curtis2023intervention}.
%However, these methods lack time sensitivity (e.g., an average of 20 minutes and 53 seconds to conduct SIC with SICG~\cite{mandel2023pilot}) and do not offer adaptive, individualized guidance tailored to the wide range of clinical conditions seen in older adult patients in the ED.  
%Moreover, these frameworks and interventions are designed to support clinicians during the conversation itself, but not for the broader clinical workflow. %%if like this, in the challenges part we need to talk about the challenges more than the conversation.
%As a result, they are unsuitable for use in the fast-paced and high-workload ED environment.


%~\citet{curtis2023intervention} explored a digital intervention (the Jumpstart Guide) to automatically extract structured patient data (ie, life-sustaining treatment preferences and chronic conditions) from the EHR and provide communication templates, which are sent by email to remind clinical care teams to initiate timely SICs. 


%%%%%% uncertainty about prognosis %%%%%%%
%Moreover, uncertainty about prognosis is also one of the concerns for clinical care teams to conduct SIC~\cite{galvin2017adverse}, which can delay SIC, slow down decision-making, and miss the opportunity for timely intervention. %%why does uncertainty about prognosis delay SIC?
%The lack of clarity about how the illness will progress, combined with concerns about upsetting the patient, can still cause clinical care teams to delay important conversations about serious illness during the early stages, even if they know the patient’s condition could become worse~\cite{shilling2024let}.



 %and met resistance from some clinical care teams~\cite{mandel2023pilot}. 
%%the challenges are not identified in the findings
However, clinical care teams barely conduct SICs in the ED. 
Research by \citet{prachanukool2022emergency} examining 332 older adult patients found that 63\% did not experience a SIC in the ED, which highlights the gap between need and practice. 
This gap stems from multiple interconnected challenges that clinical teams encounter in the unique ED settings. 
EDs can admit up to 120 patients per day~\cite{jones2008forecasting}, and this high patient volume severely limits care teams' capacity to conduct SICs with each older adult patient facing serious illness~\cite{adeyemi2024emergency}. 
Beyond time pressures, many clinical care teams struggle with uncertainty about how to appropriately initiate these sensitive conversations~\cite{ouchi2019goals}, which creates hesitation that further reduces the likelihood of SICs occurring. 
Additionally, prognostic uncertainty compounds these challenges, as clinical care teams often remain uncertain about patients' conditions and tend toward optimism about patient outcomes~\cite{christakis2000extent}.
As a result, this uncertainty can delay recognizing when SICs are needed and thus hinder their timely initiation.
Existing frameworks are designed to support clinical care teams in conducting SICs.
For example, the Serious Illness Conversation Guide (SICG) \cite{bernacki2015development} offers a structured question framework that can be used during SICs \cite{grudzen2025palliative}. 
However, SICG requires substantial time investment (an average of over 20 minutes~\cite{mandel2023pilot}) and provides static guidance that cannot adapt to the diverse, rapid-fire situations common in the ED. 
%Furthermore, these frameworks focus primarily on supporting clinicians during the conversation itself rather than integrating with the broader clinical workflow, making them poorly suited for the fast-paced, high-workload environment that characterizes emergency departments.
%and the Jumpstart Guide \cite{curtis2023intervention}


SICs are forms of patient-provider communication. 
Beyond the context of SICs, the Human-Computer Interaction (HCI) community has proposed some technical solutions that support such communication.
For example, \citet{ryu2023you} built an interactive system to record patients' care preferences, and those preferences are then shared with clinical care teams, while \citet{yang2024talk2care} designed a Large Language Model-powered system to support asynchronous communication between older adults and clinical care teams. 
However, there is limited research that focuses on exploring technological solutions to support clinical care teams' workflow of SICs in high-stakes and time-sensitive ED settings. 
Recognizing this gap, there have been increasing calls from the medical community to leverage AI technologies to support the workflow of SICs. 
%For example, \citet{manz2020effect} showed that AI-generated mortality predictions with behavioral nudges to clinical care teams can improve SIC frequency. 
For example, \citet{chua2022enhancing} proposed conversational agents (CAs) to collect patients' information and care preferences before having SIC with clinical care teams to maximize the efficiency of SICs. 
They further proposed AI to streamline the SIC documentation process~\cite{chua2022enhancing}, which could save clinical care teams' time and further increase the efficiency of SICs.




To respond to these calls, we aim to explore specific AI opportunities to better support SICs.
Although prior studies have identified barriers to conducting SICs from the clinical care teams' perspective~\cite{shilling2024let}, these findings are often described at a high level and lack the granular workflow-specific insights necessary for designing effective AI support systems.
To address the gap, our study seeks to explore two research questions (RQs):
\begin{enumerate}
\item RQ1: What challenges and needs do clinical care teams face in their workflow of conducting serious illness conversations with older adult patients in the emergency department?
\item RQ2: What design considerations should inform the development of AI tools to support clinical care teams in their workflow of conducting serious illness conversations?
\end{enumerate}
%To address these questions, we first conducted expert interviews with two clinical experts who are highly experienced in SIC in ED and also researchers in this field.
%The goal of the initial expert interviews is to better understand the workflow in conducting SIC in ED and these experts' perception of AI opportunities in supporting SIC. 


SICs in the ED are highly contextual and emergent, with no unified evidence-based workflow currently established.
Thus, we adopted a multi-phase approach (Fig. \ref{fig:workflow_ui}) to systematically understand both current practices and future opportunities for AI support. 
We began with formative expert interviews involving two highly skilled clinician-researchers, each with extensive experience in both practicing and studying SICs in the ED. 
%These interviews aimed to surface implicit workflow stages, identify variability in current practices, and explore potential AI intervention points within SIC processes. Through this initial phase, we derived a four-step workflow framework (identification, preparation, conduction, and documentation) and developed a series of text-based AI technology probes that served as concrete examples for discussing AI capabilities with practitioners. 
These interviews outline the generic SIC workflow and surfaced four stages: identification, preparation, conduction, and documentation. 
In addition, we created text-based AI technology probes based on their insights about AI.
%These probes served as concrete examples for discussing AI capabilities with clinical care teams. 
This foundational understanding informed the development of a semi-structured interview guide for subsequent interviews with nine clinical care team members working in the ED. 
The interview guide systematically aligned workflow-related questions with each stage and decision point in the SIC process, which enables us to probe clinical care teams' specific needs and challenges.
During interviews with clinical care team members who had limited familiarity with AI technologies, we utilized our text-based AI technology probes to prompt reflection on where AI might provide meaningful support.  
This process yielded design guidelines that address the unique challenges clinical care teams face when conducting SICs in the fast-paced, time-constrained ED environment. 
This paper makes the following key contributions: 

\begin{itemize}
\item \textbf{A detailed characterization of clinical care teams' workflow for conducting SICs with older adult patients in the ED}, derived from expert interviews and validated through practitioner interviews, revealing four key stages and associated challenges.

\item \textbf{An empirical analysis of the specific needs, challenges, and opportunities clinical care teams encounter at each stage of the SIC workflow}, based on interviews with nine emergency department practitioners, highlighting critical pain points in time-constrained environments.

\item \textbf{Design guidelines for AI tools supporting SICs in emergency care}, informed by practitioner feedback on where and how AI can meaningfully augment clinical workflows without disrupting patient care.

\end{itemize}


%Rationale on how is this RtD: We start with a design situation (the complexities of SICs in emergency care),
%We conduct early contextual inquiry (formative expert interviews),
%We design speculative or partial artifacts (design probes),
%We interpret clinicians’ reactions to these artifacts to develop new understanding of the design space (e.g., what AI should not do, what support is culturally/ethically appropriate, how control and empathy are negotiated).

%%AI%%%%%%%%%%%%%%%%%%%%%%%
%Recently, advanced AI technology has shown the potential to support clinical care teams in their workflow of conducting SIC~\cite{foong2024designing}. 
%For instance, Large Language Models (LLMs) hold significant promise in extracting key patient information from vast clinical data within EHRs as well as conversational information and presenting it in a cognitively accessible format for clinical care teams~\cite{wu2024cardioai}. 
%In addition, many studies explored leveraging AI prediction models to predict patients' prognosis, such as the risk of developing a specific disease~\cite{yang2019unremarkable, zhang2024rethinking} or mortality~\cite{kwon2019artificial}. 
%Meanwhile, another line of research demonstrated AI's capability to generate contextually relevant and high-quality questions based on different information~\cite{zeghouani2024examining, labutov2015deep}. 



%However, it remains underexplored whether and how these AI technologies may effectively support clinical care teams' in their workflow of conducting SIC with older adults who have serious illness in ED. 
%To better understand how we could use AI technology to build tools that support clinical care teams to conduct SIC, we need follow the Human-Centered AI principle~\cite{} to know the challenges and needs clinical care teams face in their workflow of conducting the SIC, and get them involved in the design process.
%Although existing studies have identified challenges in conducting SIC, these challenges are often described at a high level, making it difficult to generate actionable insights on how to effectively support clinical care teams and increase their confidence in conducting SICs.

%Thus, our work aims to investigate clinical experts' current workflow with respect to their challenges and needs in conducting SIC with older adult patients who have serious illnesses. 



%Conversational agents (CAs) powered by large language models (LLMs) have shown promise in engaging in natural verbal conversations within clinical settings~\cite{}. 
%HCI research demonstrates the ability of AI to extract the necessary information of patients from EHRs with greater accuracy and in a shorter time~\cite{chi2021development}, as well as the potential of presenting the extracted information in AI-powered systems for clinical experts to review~\cite{}. 


 
%Moreover, a study has demonstrated the ability of natural language processing (NLP) to process transcribed dictation and generate EHR documentation, reducing documentation time for clinical experts while maintaining document quality~\cite{kaufman2016natural}.




%The Serious Illness Conversation Guide (SICG) acts as a framework to support discussions between clinicians, patients, and their families about their illness understanding, information preferences, prognosis, key topics (i.e., goals, fears, worries, critical abilities, family involvement, etc.), and clinician recommendations~\cite{baxter2022patient}.

%_____________ downside of the framework SICG
%The original Serious Illness Conversation Guide was designed for use upstream for advance care planning, when patients are feeling well, and was not initially intended for use when patients are acutely ill, as in the ED~\cite{aaronson2021adapting}.

%Consistent with previously reported data, we met resistance from nephrologists who declined to conduct the conversations with their own patients for a variety of reasons, including lack of time and discomfort with discussing serious illness. (a pilot study in dialyss clinic settinig showed)~\cite{mandel2023pilot}.

%The original Serious Illness Conversation Guide was designed for use upstream for advance care planning, when patients are feeling well, and was not initially intended for use when patients are acutely ill, as in the ED.(maybe not suitable in ed)~\cite{aaronson2021adapting}.


%_____________ intervention for eliciting value and goal, but patients still want to talk with doctor. these tools are not for supporting clinical care teams in ed

%_____ exsitng lit call for AI to support clinical care providers in SIC. details.... but we don't know how clinical care teams perspections towards AI technology in SIC. To better understand how AI technologies can support them in SIC, we need to know their challenges and needs in their workflow of conducting SIC. Although there are already some challenges be mentioned by previous research~\cite{}. There are too broad and lack of actionable insights about how we can provide support to deal with clinical care teams' challenges. Only knowing those high level challenges are not enough to understand why the clinicians are not having the conversation. Thus, .....



%There are existing systems aimed at encouraging patients to express their values and goals and then provide this information to clinical experts as evidence to make their clinical decisions...
%value ecilitatioon tool + communication tools + visualization tool

%, as many patients still prefer to engage in SIC with their physicians in person~\cite{chua2022enhancing}. 
%Moreover, even when clinical experts utilize data from these tools, they need to manually extract and input the information into the EHR systems~\cite{}—a time-consuming task that can discourage further processing.

%Despite some SICs being documented in EHR systems, ~\citet{chandar2017perspectives} found that the information of SICs provided to clinical experts remains inconsistent.








%If patients later lose the ability to express their preferences, their family needs to make clinical decisions for them. 
%In many cases, there is a misalignment between what the family wants and what the patient would have chosen~\cite{kitzinger2018deaths}, which increases the likelihood that patients will receive care that does not reflect their values or preferences.


%while families face overwhelming medical decisions without clear guidance, leading to distress, regret, and prolonged emotional suffering~\cite{}.


%%——————————————time constrain
%Addressing the complex care needs of older adults in an ED setting is expected to place increased strain on a system that is already burdened with overcrowding.(8-10)~\cite{latham2014emergency}.


%______hard to find SIC in EHR (for the intervention?)
%Goals of care documentation (Physician Orders for Life-Sustaining Treatment (POLST)/GOC note/advanced directive) may be hard to find in the medical record,14–18~\cite{bigelow2024difficult}.

%More than 70\% of these patients express priorities focused on comfort and quality of life rather than life extension [20], yet a systematic review revealed that 56–99\% do not possess advance directives in the ED [21], and many are at risk of receiving care that does not align with their goals [22].~\cite{prachanukool2022emergency}.

%Even if ACP occurred before ED arrival, it is rarely recorded in the medical records15 and patients’ values and goals may change based on changing health states necessitating ED physicians revisiting patients’ goals~\cite{fried2007inconsistency}.
%prognosis

%Goals of care documentation may be hard to find in the medical record,14–18~\cite{bigelow2024difficult}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% V1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Serious illness conversations (SIC) are a special case of patient-provider communication in critical care situations (e.g., ED and ICU), where the care provider team discusses with patients or their caregivers about the patient's goals and values of care and life~\cite{}. 
% % Serious illness conversations (SIC) are conversations between clinical experts and patients with serious illnesses~\cite{sanders2020quality} (i.e., cancer and cardiovascular diseases~\cite{hamidpour2014summer}). %and Alzheimer’s
% SIC are of significant importance to seriously ill patients because many patients 
% Care providers are expected to elicit patient's values, goals, and preferences related to their health and medical care so that they can better align the critical clinical decisions (e.g., treatment plans) with the patient's wishes and priorities of care and life
% % SIC is conducted to elicit patients' values (the most important things in their lives), care goals, and treatment preferences 
% % from patients with serious illness at the end of their lives
% ~\cite{paladino2023improving, hachem2025electronic}.

% SICs are commonly conducted among older patients because this population faces a higher likelihood of serious or life-limiting illnesses, is statistically closer to the end of life, and has more complex clinical decision-making needs~\cite{}.
% % Among patients who have SIC with clinical experts, older adults form the largest group. 
% Studies have shown that during the last six months of life, 75\% of older adults visit hospitals with preexisting serious illnesses, such as advanced heart failure, lung disease, and cancer~\cite{}.
% % Each year in the U.S., approximately xx of older adults are diagnosed with a serious illness, and most of them are in the Emergency Department (ED)~\cite{}.
% Further, older adults often have multiple comorbidities, and the clinical team often relies on SIC to improve the quality of care for patients with complicated clinical decision-making needs and life-limiting illnesses~\cite{}.
% % Conducting SIC is important because it guides clinicians to make proper clinical decisions and care planning that aligns with patient values and goals in an emergency~\cite{geerse2019qualitative, paladino2023improving, hachem2025electronic}. 
% % In this way, patients don't need to suffer from unnecessary medical treatment (i.e., being put on a ventilator), leading to discordance between patient desires and the actual care delivered and increasing patients' quality of life~\cite{}. 
% %These values and goals are especially critical among patients who have serious illnesses, as they significantly influence clinical experts' decision-making about treatment~\cite{} and the development of a goal-concordant care plan in a patient's final stage of life~\cite{geerse2019qualitative}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% V4 ED-Older Adults %%%%%%%%%%%%%%%%%%%%%%%
%SIC are especially important in the Emergency Department (ED) environment.
%ED often serves as an entry point to the hospital system~\cite{ouchi2019goals}, and conducting SIC at this point may help guide the entire treatment trajectory that provides patient-centered care. 
%Among all ED visits, older adult patients aged $\geq 65$ years account for one-quarter of the visits~\cite{} and often arrive during a critical turning point in their serious illness trajectory~\cite{}.
%Studies show that 50\% of older adults visit the ED in the last month of life, and 75\% do so within six months of death~\cite{wilson2020end}.
%Conducting SIC with older adult patients helps clinical care teams to make high-stakes decisions under time pressure.
%Moreover, SIC help older adult patients... 
%Without SIC, older adult patients may obtain default and unwanted aggressive treatment, such as chemotherapy, ventilation, or intubation~\cite{wright2008associations}, which can increase patients’ suffering and reduce their quality of life in their last stage of life~\cite{wright2008associations}.
%For example, if older adult patients experience an intubation (a tube into the airway), they can experience sensations of suffocation~\cite{knudsen2015awake}, which may be hard for them to handle physically and psychologically.
%but also become increasingly aggressive over time~\cite{wright2008associations},
%Moreover, aggressive treatments are often associated with nearly double the healthcare costs compared to the non-aggressive approaches~\cite{teno2002medical}, which can place a significant financial and emotional burden on already seriously ill older adult patients and their families. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%which leads to the increase of patients' satisfaction and quality of life~\cite{bernacki2019impact, wright2008associations}.
%Older adult patients who visit ED normally are in an inflection point in their illness trajectory, portending a worsening course~\cite{ouchi2019goals}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%SIC is important for both clinical care teams and patients with serious illness.
%SIC can guide the clinical care teams to make patient-centered clinical decisions~\cite{}, which leads to goal-concordant care~\cite{geerse2019qualitative}. 
%In this way, serious illness patients are less likely to receive unwanted or non-beneficial treatments and experience reduced anxiety and depression~\cite{detering2010impact}, thereby achieving a better quality of life.~\cite{bernacki2019impact, wright2008associations}.
%Without SIC, older adult patients may obtain default and unwanted aggressive treatment, such as chemotherapy, ventilation, or intubation~\cite{wright2008associations}. 
%For example, if patients experience an intubation (a tube into the airway), they can experience sensations of suffocation~\cite{knudsen2015awake}, which may be hard for them to handle physically and psychologically.
%but also become increasingly aggressive over time~\cite{wright2008associations},
%Moreover, these aggressive treatments are often associated with higher healthcare costs~\cite{teno2002medical}, which can place a significant financial and emotional burden on already seriously ill patients and their families. 











%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% V2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%SIC is particularly important for older adult patients aged $\geq 65$ years with serious illness in Emergency Department (ED) environments.
%ED is a common site of access to care for older patients with serious illness~\cite{wilson2020end} and often serves as an entry point to the hospital system~\cite{ouchi2019goals}. 
%Among ED visits, older adult patients account for up to a quarter of all the visits~\cite{samaras2010older}, totaling 156 million visits in the U.S.~\cite{pines2013national}.
%This population is also more likely to experience a gradual decline in health and an increased likelihood of ED visits due to functional deterioration.
%and is often in closer proximity to the end of life~\cite{raj2019older, cook2014making}. 
%A study showed that 50\% of older adults visit the ED in the last month of life in the U.S., and 75\% visit the ED within six months of their death~\cite{wilson2020end}.
%In this high-risk and high-stake ED environment, 
%For older adult patients with serious illness, SIC is associated with lower rates of in-hospital death, earlier hospice referrals, increased peacefulness, and a greater likelihood to have a high quality of end-of-life~\cite{prachanukool2022emergency}. 
%beneficial for decreasing the risk of treatment burdens that may outweigh the benefits, which ultimately improves care quality and reduces psychological distress for both patients and their families~\cite{back2019serious, wright2016family}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% V1 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Serious illness conversations (SIC) are a special case of patient-provider communication in critical care situations (e.g., ED and ICU), where the care provider team discusses with patients or their caregivers about the patient's goals and values of care and life~\cite{}. 
% % Serious illness conversations (SIC) are conversations between clinical experts and patients with serious illnesses~\cite{sanders2020quality} (i.e., cancer and cardiovascular diseases~\cite{hamidpour2014summer}). %and Alzheimer’s
% SIC are of significant importance to seriously ill patients because many patients 
% Care providers are expected to elicit patient's values, goals, and preferences related to their health and medical care so that they can better align the critical clinical decisions (e.g., treatment plans) with the patient's wishes and priorities of care and life
% % SIC is conducted to elicit patients' values (the most important things in their lives), care goals, and treatment preferences 
% % from patients with serious illness at the end of their lives
% ~\cite{paladino2023improving, hachem2025electronic}.

% SICs are commonly conducted among older patients because this population faces a higher likelihood of serious or life-limiting illnesses, is statistically closer to the end of life, and has more complex clinical decision-making needs~\cite{}.
% % Among patients who have SIC with clinical experts, older adults form the largest group. 
% Studies have shown that during the last six months of life, 75\% of older adults visit hospitals with preexisting serious illnesses, such as advanced heart failure, lung disease, and cancer~\cite{}.
% % Each year in the U.S., approximately xx of older adults are diagnosed with a serious illness, and most of them are in the Emergency Department (ED)~\cite{}.
% Further, older adults often have multiple comorbidities, and the clinical team often relies on SIC to improve the quality of care for patients with complicated clinical decision-making needs and life-limiting illnesses~\cite{}.
% % Conducting SIC is important because it guides clinicians to make proper clinical decisions and care planning that aligns with patient values and goals in an emergency~\cite{geerse2019qualitative, paladino2023improving, hachem2025electronic}. 
% % In this way, patients don't need to suffer from unnecessary medical treatment (i.e., being put on a ventilator), leading to discordance between patient desires and the actual care delivered and increasing patients' quality of life~\cite{}. 
% %These values and goals are especially critical among patients who have serious illnesses, as they significantly influence clinical experts' decision-making about treatment~\cite{} and the development of a goal-concordant care plan in a patient's final stage of life~\cite{geerse2019qualitative}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






%%%%________why SIC?
%positive
%patients who receive have SIC, their the medical treatment aligns more with their goals and values, their family have much more lower stress, anxiety level and depression level.~\cite{detering2010impact}

%nagetive-consequence without SIC
%Aggressive care is associated with worse patient quality of life and worse bereavement adjustment.
%more aggressive medical care was associated with worse patient quality of life and higher risk of major depressive disorder in bereaved caregivers. Patients who received aggressive medical interventions had worse quality of life in the final week of life. Patients' quality of life decreased with increasing numbers of aggressive medical therapies~\cite{wright2008associations}.



==> sections/draft_introduction_v2.tex <==
\section{Introduction}

%why matters to older adults; Aritifical (AI), put citations toghether, design opportunities; make clear about the goals of the paper; the definition of goal-aligned care; 

%% OLD PARAGRAPH 1 - COMMENTED OUT
%Older adults (aged 60 and above) comprise up to a quarter of all emergency department (ED) visits~\cite{samaras2010older}, with many presenting life-threatening illnesses such as heart failure or advanced cancer~\cite{smith2012half}.
%In 2017, 29 million older adults (aged 60 and above) visited the emergency department (ED)~\cite{ashman2020emergency}.
%To save these patients' lives, healthcare providers often resort to aggressive treatment~\cite{dzeng2018homing, gips2022palliative}, such as intubation and mechanical ventilation~\cite{wright2008associations}. 
%Although these treatments may temporarily extend life, they frequently impose significant burdens on patients~\cite{ gleason2003delirium, bassi2021systematic, knudsen2015awake, Rubin_Buehler_Halpern_2016}, including severe pain~\cite{yamashita2017risk}, memory difficulties~\cite{shehabi2010delirium}, and independent breathing capacity~\cite{jubran2019long}.
%These side effects may discourage patients from pursuing aggressive treatments.
%In one study of 340 older adult patients with life-threatening illnesses, 64\% preferred not to be connected to machines, and 93\% prioritized being free from pain~\cite{steinhauser2000factors}.
%However, patients may receive care that conflicts with their goals of care~\cite{teno2002medical}, which results in unnecessary suffering and diminished quality of life~\cite{wright2008associations}.
%This misalignment underscores a critical need for healthcare providers to understand patients' goals of care before making clinical decisions.

%% NEW PARAGRAPH 1 - Define Hard Conversations/SICs with Vivid Example  
Healthcare providers need to understand patients' goals of care when treating life-threatening illnesses. Serious Illness Conversations (SICs) serve as essential patient-provider communications for this purpose~\cite{ouchi2017preparing, peloquin2025discussions}. 
Consider a scenario where an elderly heart failure patient arrives unconscious at the emergency department (ED): healthcare providers must engage with family members to discuss whether to place the patient on a ventilator~\cite{wright2008associations} or transition to comfort care.
Although aggressive treatments may temporarily extend life, they frequently impose significant burdens~\cite{gleason2003delirium, bassi2021systematic, knudsen2015awake, Rubin_Buehler_Halpern_2016}, including severe pain~\cite{yamashita2017risk}, memory difficulties~\cite{shehabi2010delirium}, and loss of independent breathing capacity~\cite{jubran2019long}.
Through SICs, healthcare providers systematically explore patient preferences: they discuss expected disease trajectory~\cite{ouchi2017preparing}, uncover fundamental values (e.g., the desire to be alive for grandchildren~\cite{naik2016health}), clarify goals of care (e.g., curative treatment versus comfort care), and identify specific treatment preferences~\cite{shilling2024let}.
In one study of 340 older adult patients with life-threatening illnesses, 64\% preferred not to be connected to machines, and 93\% prioritized being free from pain~\cite{steinhauser2000factors}, yet patients may receive care that conflicts with their goals~\cite{teno2002medical}, resulting in unnecessary suffering~\cite{wright2008associations}.
SICs allow providers to deliver care that minimizes suffering, offers emotional support, and preserves quality of life~\cite{prachanukool2022emergency, ouchi2017preparing, geerse2019qualitative}.

%% NEW PARAGRAPH 2 - Current Practice Gap + Older Adult Focus
Currently, SICs typically occur in ICUs and post-emergency settings, where patients have already been admitted and clinical decisions such as ICU admission or certain treatments have been performed~\cite{ouchi2019goals}. 
However, SICs are rarely conducted in EDs, which often serve as the primary entry point into the hospital system~\cite{ouchi2019goals}, and initial treatment plans are formulated~\cite{wilson2020end}. 
This absence is particularly concerning for older adults (aged 60 and above), who comprise up to a quarter of all ED visits~\cite{samaras2010older, galvin2017adverse} and often present with life-threatening illnesses such as heart failure or advanced cancer~\cite{smith2012half}.
One study involving 332 older adult patients revealed that more than half had not received a SIC during their ED visit~\cite{prachanukool2022emergency, ouchi2019goals, clark2018racial}, and many of them lack documented treatment goals and care preferences~\cite{ouchi2017preparing}.
Prior research suggests that SICs are often not conducted in EDs due to several barriers: clinicians may face time constraints and high patient turnover, which limit their ability to engage in lengthy conversations~\cite{ouchi2019goals, clark2018racial}. 
Additionally, the unpredictable and fast-paced nature of the ED environment can make it challenging to prioritize SICs~\cite{wilson2020end}. Furthermore, some clinicians may feel inadequately trained to handle the emotional and complex nature of these conversations, leading to reluctance in initiating them~\cite{shilling2024let}.


%% NEW PARAGRAPH 3 - Evidence for Early ED Conversations - The "Yet" Contradiction
Yet prior research demonstrates that conducting SICs early in the ED can lead to significant benefits for older adults~\cite{prachanukool2022emergency}.
For high-risk, clinically unstable, and vulnerable older adults in the ED, conducting SICs can lead to less aggressive medical care near the end of the patient's life (e.g., mechanical ventilation or resuscitation), reduce stress among surrogates, and a higher likelihood that care aligns with patients' wishes~\cite{ouchi2017preparing}.
When patients receive care that aligns with their goals, they experience higher satisfaction with their care~\cite{ouchi2017preparing} and optimized quality of their end-of-life experiences~\cite{geerse2019qualitative}.
Some practitioners have begun advocating for this approach~\cite{paladino2023improving, hachem2025electronic}, recognizing that EDs represent a critical moment to understand patients' goals and values for delivering goal-concordant care, given that half of older adult patients in the ED are in the last month of life, and three-fourths are within six months of their death~\cite{wilson2020end}.

%% NEW PARAGRAPH 4 - Study Focus and Research Questions
While SICs involve diverse family dynamics across different patient populations, this paper focuses on older adult patients as a case study to explore the fundamental question: how could healthcare providers conduct SICs in EDs, and why they may not want to do so?
Although previous research identified some barriers in SICs~\cite{geerse2019qualitative, shilling2024let}, most have been studied outside ED settings and rarely probe into their underlying causes~\cite{ouchi2019goals}.
Without a clear understanding of SIC workflow in the ED and the specific challenges healthcare providers face, it is difficult to develop effective solutions.
Therefore, our study asks the first research questions (RQ):
\begin{enumerate}
\textbf{RQ1:} How do healthcare providers approach conducting SICs with older adults in emergency departments, and what are their motivations and barriers toward engaging in these conversations?
\end{enumerate}

%% NEW PARAGRAPH 5 - AI as Secondary Context
The challenge of supporting patient-provider communication has garnered increasing attention within the Human-Computer Interaction (HCI) community, with researchers exploring various technology-mediated solutions~\cite{ramesh2024data, patel2013visual, jang2014bodydiagrams, ni2011anatonme, bascom2024designing, jo2024exploring, liaqat2024promoting, wang2024commsense, berry2019supporting, yang2024talk2care, chen2025designing}.
However, existing HCI research has mainly focused on communication scenarios that are less time-constrained and emotionally intensive than those encountered in emergency care.
Recent advances in AI technology offer promising new avenues to address these specific challenges and support healthcare providers in conducting SICs within the demanding ED environment.
AI risk prediction models have demonstrated capability in forecasting patient mortality rates~\cite{kwon2019artificial, pourhomayoun2020predicting, avati2017improving, wang2019development}, which could potentially help providers identify which patients would most benefit from SICs~\cite{manz2020effect}. 
Beyond risk stratification, Large Language Models (LLMs) show promise in generating contextually appropriate, condition-specific questions~\cite{maity2024future, yang2024talk2care} and providing emotional support~\cite{zheng2025customizing, seo2025enhancing, kumar2023exploring}.
Recognizing these potential benefits, the medical community has begun advocating for the systematic integration of AI into SIC workflows~\cite{chua2022enhancing}.
Therefore, we ask the second research question:
\begin{enumerate}
\textbf{RQ2:} What technological opportunities, particularly AI-driven solutions, can be designed to support healthcare providers in their SIC workflow in the ED settings?
\end{enumerate}



%% OLD PARAGRAPHS - COMMENTED OUT
%%Older adults (aged 60 and above) comprise up to a quarter of emergency department (ED) visits~\cite{samaras2010older}, with many presenting life-threatening illnesses such as heart failure or advanced cancer~\cite{smith2012half}. When treating these critically ill patients, healthcare providers often resort to aggressive interventions such as intubation and mechanical ventilation~\cite{dzeng2018homing, gips2022palliative, wright2008associations}. Although these treatments may temporarily prolong life, they come with significant burdens, including severe pain~\cite{yamashita2017risk}, memory difficulties~\cite{shehabi2010delirium}, and loss of independent breathing capacity~\cite{jubran2019long} that can persist long after treatment~\cite{gleason2003delirium, bassi2021systematic, knudsen2015awake, Rubin_Buehler_Halpern_2016}.Given these serious side effects, many older adults prefer to avoid such aggressive care. In fact, one study of 340 older adult patients with life-threatening illnesses found that 64\% preferred not to be connected to machines, and 93\% prioritized being free from pain~\cite{steinhauser2000factors}. Yet despite these preferences, patients often receive care that conflicts with their goals~\cite{teno2002medical}, resulting in unnecessary suffering and diminished quality of life~\cite{wright2008associations}. This disconnect highlights the critical need for healthcare providers to understand patients' goals of care before making clinical decisions.

%%To understand patients' goals of care, Serious Illness Conversations (SICs)~\cite{ouchi2017preparing}, a form of patient-provider communication initiated when patients have a life-threatening illness, are essential~\cite{peloquin2025discussions}. 
%%Through SICs, healthcare providers systematically explore multiple dimensions of patient preferences: they discuss patients' expected disease trajectory~\cite{ouchi2017preparing}, uncover patients' fundamental values (e.g., the desire to be alive for grandchildren~\cite{naik2016health}), clarify goals of care (e.g., curative treatment versus comfort care), and identify specific treatment preferences(e.g., intubation versus pain management) regarding interventions~\cite{shilling2024let}.
%%When conducting SICs with older adults who prioritize comfort care, SICs allow providers to deliver care that minimizes suffering, offers emotional support, and preserves quality of life.~\cite{prachanukool2022emergency, ouchi2017preparing, geerse2019qualitative}.


% =============== where Dakuo stops ===============


Despite the demonstrated value of SICs, healthcare providers often do not conduct SICs~\cite{ouchi2019goals, clark2018racial}.
Research involving 332 older adult patients revealed that more than half had not received a SIC during their ED visit~\cite{prachanukool2022emergency}.
Healthcare providers often face multiple challenges conducting SICs~\cite{geerse2019qualitative}.
First, healthcare providers may face uncertainty regarding a patient’s prognosis, making it difficult to identify those who need SICs~\cite{shilling2024let}. 
%Moreover, older adult patients may arrive at the ED unconsciously (e.g., coma)~\cite{acar2024problem} with no family around~\cite{han2013altered}, which makes it impossible for healthcare providers to conduct SICs. 
%While providers can review patients' care preferences through the electronic health record (EHR), more than half of patients may lack such documentation~\cite{oulton2015advance}.
Even when appropriate patients are identified, many healthcare providers hesitate to initiate SICs due to insufficient training in SIC skills~\cite{ouchi2019goals}. 
This reluctance is further amplified by providers' concerns about delivering distressing prognostic information, as many fear that discussing limited life expectancy may cause significant emotional harm to patients~\cite{shilling2024let}.
To address these barriers, researchers developed the SIC Guide (SICG), which offers structured, pre-written questions to facilitate SICs~\cite{bernacki2015development}.
However, the SICG's lengthy duration (approximately 22 minutes per SIC~\cite{mandel2023pilot}) creates practical constraints that limit its feasibility in the fast-paced ED environment.




The challenge of supporting patient-provider communication has garnered increasing attention within the Human-Computer Interaction (HCI) community.
To rise to the challenge, researchers have explored various technology-mediated solutions to support such communication~\cite{ramesh2024data, patel2013visual, jang2014bodydiagrams, ni2011anatonme, bascom2024designing, jo2024exploring, liaqat2024promoting, wang2024commsense, berry2019supporting, yang2024talk2care, chen2025designing}.
For example, ~\citet{ramesh2024data} designed a web-based tool for healthcare providers to review patients’ progress through staged rehabilitation assessments.
Moreover, ~\citet{patel2013visual} that leverages visual feedback to improve provider communication performance.
However, existing HCI research has mainly focused on communication scenarios that are less time-constrained and emotionally intensive than those encountered in emergency care.
However, there remains a research gap in understanding how to leverage technology to support healthcare providers in conducting SICs within the demanding context of emergency care.




Recent advances in AI technology offer promising new avenues to address these challenges and support healthcare providers in conducting SICs within the ED environment.
AI risk prediction models have demonstrated capability in forecasting patient mortality rates~\cite{kwon2019artificial, pourhomayoun2020predicting, avati2017improving, wang2019development}, which could potentially help providers identify which patients would most benefit from SICs~\cite{manz2020effect}. 
Beyond risk stratification, Large Language Models (LLMs) show promise in generating contextually appropriate, condition-specific questions (e.g., personalized health check-in inquiries tailored to individual patient circumstances)~\cite{maity2024future, yang2024talk2care}, which may support healthcare providers in initiating SICs based on patients' health conditions.
Moreover, LLMs have been explored as tools for providing patients with emotional support (e.g., showing empathy, comforting patients and their family, and providing positive guidance)~\cite{zheng2025customizing, seo2025enhancing, kumar2023exploring}.
Recognizing these potential benefits brought from AI, the medical community has begun advocating for the systematic integration of AI into SIC workflows~\cite{chua2022enhancing}. 
For example, they proposed leveraging conversational agents (CAs) to elicit patients' care preferences.
Moreover, they advocate for using AI to streamline the documentation of SICs.




Despite these promising technological capabilities, there remains a limited understanding of how AI technologies can support healthcare providers in conducting SICs in the time-critical ED settings.
Addressing this gap requires first developing a deeper, more nuanced understanding of healthcare providers' specific challenges and needs in SICs.
%Although older adults are stakeholders in SICs, their vulnerability could make participation in a research study inappropriate, as such engagement could heighten emotional distress and impose undue burden during a fragile stage of life.
Although older adults are stakeholders in SICs, our study did not include them as participants because our focus is on designing technologies to support healthcare providers, and these technologies are not intended to interact directly with patients.
Previous research identified some barriers in SICs (e.g., difficulties in identifying patients who need SICs, initiating and conducting SICs)~\cite{geerse2019qualitative, shilling2024let}.
However, most of these barriers have been studied outside the ED settings.
Moreover, these barriers are scattered across different phases of SICs (before and during SICs), and rarely probe into their underlying causes.
Without a clear understanding of SIC workflow in the ED, challenges and needs specific to the ED, and the causes that create challenges, it is difficult to explore how AI could support healthcare providers in real-world practice.



Therefore, our study seeks to explore two research questions (RQs):
\begin{enumerate}
\item RQ1: What challenges and needs do healthcare providers face in their workflow of conducting SICs with older adult patients in the emergency department?
\item RQ2: What design considerations should inform the development of AI systems to support healthcare providers in their workflow of conducting SICs?
\end{enumerate}



To explore these RQs, we adopted a two-stage study (Fig. \ref{fig:two_stage}).
We first began with the expert interviews to analyze their workflow for conducting SICs.
The reason for analyzing their workflow is that there is a lack of a standard and evidence-based SIC workflow in the ED.
Without understanding healthcare providers' workflow of SICs, it is hard to explore AI opportunities to support them in real-world practice.
The expert interviews involved two clinician-researchers with extensive experience both practicing SICs in the ED and training other providers to properly conduct SICs.
The results from the expert interviews outlined a standard ED-specific workflow of conducting SICs, including four stages: identification, preparation, conduction, and documentation. 
The understanding of their workflow informed the development of a semi-structured interview protocol for subsequent interviews with nine healthcare providers working in the ED. 
We then further investigated their specific needs and challenges in each stage of their workflow, as well as their perceptions on leveraging AI to support them.
The findings yielded design guidelines that address the key challenges and needs healthcare providers face when conducting SICs in the fast-paced, time-constrained ED environment. 



To the best of our knowledge, prior HCI research on technology-supported patient–provider communication has predominantly focused on non-acute, routine clinical contexts involving less sensitive conversations.
In contrast, our work contributes novel insights by identifying AI opportunities that support healthcare providers in conducting highly sensitive conversations with patients in time-critical care settings.
Our work makes the following key contributions: 

\begin{itemize}
\item \textbf{A detailed characterization of healthcare providers' workflow for conducting SICs with older adult patients in the ED}, derived from expert interviews and validated through practitioner interviews, revealing four key stages and associated challenges.

\item \textbf{An empirical analysis of the specific needs, challenges, and opportunities healthcare providers encounter at each stage of the SIC workflow}, based on interviews with nine emergency department healthcare providers, highlighting critical pain points in time-constrained environments.

\item \textbf{Design guidelines for AI systems supporting SICs in emergency care}, informed by healthcare providers' feedback on where and how AI can meaningfully augment clinical workflows without disrupting patient care.

\end{itemize}



==> sections/draft_related_work.tex <==
\section{Related Work}

\subsection{Serious Illness Conversations With Older Adult Patients in Emergency Department}

Older adult patients with serious illness face a high risk of mortality and often experience reduced quality of daily functioning and overall quality of life~\cite{kelley2018identifying}.
According to a survey, three-quarters of older adults aged 65 and older live with at least one type of serious illness~\cite{statista2022serioushealth}.
For this population, conducting SICs is essential to enable treatment plans that align with patients' values, goals, and care preferences~\cite{houben2014efficacy,silveira2010advance}.
However, many older adults have never participated in SIC~\cite{prachanukool2022emergency}, and up to 99\% lack any documented goals or values in their EHR~\cite{ouchi2017preparing}.
%Even among those who had SIC, their care preferences can naturally evolve over time~\cite{kim2016natural}. 
This combination of low SICs uptake and incomplete documentation can impede patient‑centered care and increase the frequency and duration of unnecessary hospitalizations~\cite{klingler2016does}.
Therefore, there is a pressing need to conduct SICs.




Conducting SICs with older adults in the ED environment is especially important~\cite{prachanukool2022emergency}.
Many initial treatment plans are formulated in the ED as the ED often serves as the primary entry point into the hospital system~\cite{ouchi2019goals}.
Thus, integrating SICs at this stage and conducting them effectively can profoundly influence patients’ care trajectories (i.e., ICU admission to hospice referral)~\cite{wilson2020end}.
Among all ED visits, older adults account for approximately one-quarter of the visits~\cite{galvin2017adverse}, and half of the older adult patients in the ED are in the last month of life, and three-fourths are within six months of their death~\cite{wilson2020end}.
%This population typically faces an average mortality rate of 10\%, along with a 24\% rate of ED revisits and hospital readmissions~\cite{aminzadeh2002older}.  
For high-risk, clinically unstable, and vulnerable older adults in the ED, conducting SICs can lead to less aggressive medical care near the end of the patient's life (e.g., mechanical ventilation or resuscitation), reduce stress among surrogates, and a higher likelihood that care aligns with patients’ wishes~\cite{ouchi2017preparing}.




However, healthcare providers rarely conduct SICs, with less than one-third of older adults engaged in SICs~\cite{clark2018racial}. 
Healthcare providers face significant challenges in conducting SICs.
One major challenge is that healthcare providers often have substantial time constraints in the ED~\cite{chandar2017perspectives}.
%Especially in the ED environment, where the mean length of stay per patient is only four hours~\cite{ouchi2019goals}, clinical care teams have limited capacity to engage in lengthy, emotionally charged conversations.
For example, some physicians and nurses in the ED reported high workloads and understaffing, which limited their ability to engage in lengthy, emotionally charged conversations~\cite{adeyemi2024emergency}.
In addition, healthcare providers often lack a clear, actionable protocol for initiating SICs~\cite{ouchi2019goals}, which can leave them unsure how to begin and worried that broaching the topic might trigger negative emotional responses from patients.
Furthermore, healthcare providers are sometimes uncertain about prognosis and tend to err on the side of optimism, which can delay SICs and, ultimately, critical clinical decision-making~\cite{christakis2000extent}.
%Since clinical care teams are optimistic, patients often internalize that view and choose aggressive, low‑value interventions instead of more appropriate palliative care~\cite{christakis2000extent}.



Several frameworks and programs have been developed to support conducting SICs.
SICG is the widely validated framework to provide open-ended questions to help clinical teams navigate SICs~\cite{bernacki2015development}.
%It provides a structured sequence of open-ended questions across five stages—set-up (assess, share, explore, and close) to help clinical teams navigate the SIC.
In parallel, the Serious Illness Care Program (SICP) introduces communication training and embeds reminders to improve both the quality and frequency of SICs~\cite{paladino2020training, paladino2023improving}. 
However, the framework and the program reveal notable usability and implementation gaps.
In terms of SICG, care providers required a long time to complete the SIC (20 minutes and 53 seconds)~\cite{mandel2023pilot}, which may be impractical to implement in the time-constrained ED.
%Moreover, the questions in SICG are fixed and non-adaptive, thus lacking the flexibility to accommodate the different clinical contexts and diverse individual health conditions.
As for SICP, it includes many components, but not all of them are necessary in the time-constrained setting of the ED.
%provides limited support in helping clinical care teams navigate emotional burdens during SICs~\cite{paladino2023improving}.



The ineffectiveness of the aforementioned interventions suggests a need for exploring novel approaches to support healthcare providers in their workflow of conducting SICs in the ED. 
To better support them, it is essential to understand their workflow, as well as the needs and challenges healthcare providers face in their workflow. 
However, there is limited research on these aspects.
Thus, these gaps raise the RQ1 in this paper.  






\subsection{Technological Interventions in Supporting Patient-Provider Communications}

A lot of HCI studies have focused on patient-provider communication in the past few years.
Patient-provider communication plays a crucial role in providing patient-centered care~\cite{sunnerhagen2013enhancing}, enhancing patient engagement in their care process~\cite{butz2007shared}, reinforcing positive future expectations~\cite{wright2004doctors}, and improving their mental health status~\cite{wong2019associations}. 
To better support patient-provider communication, various technological interventions have been explored~\cite{ryu2023you, ramesh2024data, seljelid2021digital, ryu2023you, bascom2024designing}. 
In addition, ~\citet{cox2025mobile} designed a mobile application to support patients’ families in providing better care by delivering guidance and information from ICU healthcare providers.
%Moreover, ~\citet{bascom2024designing} designed a set of communication feedback tools (data-driven feedback, real-time digital prompts, and guided reflection) to provide primary care physicians with personalized and actionable feedback on potential implicit biases in their patient interactions, which aims to improve communication effectiveness and promote more equitable healthcare delivery.
%%check this%%
\citet{ryu2023you} built an interactive system to record patients' care preferences, and those preferences are then shared with healthcare providers.


Another line of research explored technologies to help healthcare providers elicit patients' care preferences and goals of care~\cite{sudore2017effect, berry2021supporting, curtis2023intervention}.
For example, Living Voice is an online website to help patients document their care preferences (i.e., whether they receive mechanical ventilation or feeding tubes), and the result can be shared online with healthcare providers~\cite{vitaldecisions_mylivingvoice}. 
~\citet{foong2024designing} designed five value-elicitation prototype tools to elicit patients' values and goals through their informal caregivers. 
%In addition, researchers explored technologies to support clinical care teams in conducting SIC.
%For example, ~\citet{curtis2023intervention} explored a digital intervention (the Jumpstart Guide) to automatically extract structured patient data (e.g., chronic conditions and life-sustaining treatment preferences) from the EHR, and then provide the SIC templates to clinical care teams through emails. 
These tools are typically designed for low-pressure care settings.
In these settings, patients have more time to reflect on their care preferences and goals with healthcare providers to make decisions without urgency. 
In contrast, the ED is a high-stakes and time-constrained environment.
Older adults in the ED may experience sudden health deterioration, which makes it critical to conduct SICs to guide the treatment plans.




Recent advancements in AI present promising pathways to support healthcare providers in streamlining communication and sharing decisions~\cite{bartle2022second, li2024beyond}.
%A lot of research explored using AI-powered Conversational Agents (CAs) to support patient-provider communication.
%talk about the exmaples that mentioned in the intro in mroe detail
For instance, ~\citet{yang2024talk2care} introduced a home-based telehealth application system (Talk2Care) utilizing Large Language Models (LLMs) to support asynchronous communication between older adults and healthcare providers. 
Moreover, ~\citet{seo2025enhancing} designed an AI-based chatbot as a facilitator to fill the communication gaps between child patients, healthcare providers, and patients' parents during the clinical visits. 
%The system allows older patients to collect health information through voice, while healthcare providers can access a dashboard that summarizes and highlights key information from patient voice-assisted conversations.
%Moreover, a GPT–4–powered chatbot system was created and assessed to improve pre-visit workflows by collecting patient health information and generating interactive summaries to support clinical care teams~\cite{li2024beyond}.
%Another line of research focuses on using AI to streamline communication and share decisions in clinical settings~\cite{bartle2022second}. 
In addition, ~\citet{hao2024advancing} built an AI system that supports older adult cancer patients in expressing their preferences, raising questions, and engaging in treatment decision discussions with their cancer care clinicians during consultations. 
Although these studies explored AI in supporting patient-provider communication, few of them have examined using AI-based tools to support healthcare providers in SICs with older adult patients in the ED environment.
To bridge the gap, our work aims to explore the AI opportunities in this unique and important scenario.







\subsection{AI Technologies in Supporting the SICs}
%%%%calls from healthcare 
Current research explored some AI-based solutions to support clinicians in their workflow of conducting SICs.
For example, one group of researchers developed an AI algorithm to predict patients’ mortality rates. 
The mortality rate helps clinicians save a large amount of time in identifying high-risk patients~\cite{avati2018improving} and conduct the SIC with them. 
Another group of researchers increased the frequency of conducting the SIC by sending the message of AI mortality risk predictions and a reminder about considering initiating SICs to oncology clinicians~\cite{manz2020effect}.
In addition, Hachem et al.~\cite{hachem2025electronic} developed a dashboard to help track clinicians’ SICs training progress and facilitate documentation of the SICs.
Moreover, researchers explored the potential of using natural language processing to help healthcare providers find information on previous SICs in patients' EHRs~\cite{lindvall2022natural}. 
%For example, one study developed a method that integrates NLP and ML to identify the documentation of the SIC within 3,183 clinical notes~\cite{lee2021identifying}.



Another line of research proposed an AI-human collaborative workflow for conducting the SIC~\citet{chua2022enhancing}.
Before the SIC, they suggested using CAs to collect the needed patients' information to better prepare for SICs.
After the SIC, they highlighted the potential of using NLP to improve both the efficiency and quality of SICs documentation.
Given AI's potential to evaluate communication skills in clinical settings~\cite{ryan2019using}, they also proposed leveraging AI to analyze previous SICs and provide feedback to healthcare providers.
Although there are calls and research on leveraging AI to support healthcare providers in conducting SICs, we still have a limited understanding of whether and how healthcare providers want AI to support them, especially in the high-stakes, high-risk, and time-constrained ED environment. This gap becomes the foundation to validate the RQ2 in this paper. 













==> sections/draft_semi_structured_interviews.tex <==


\section{Interviews with Healthcare Providers Working in the ED}
Based on the formative expert interviews, we identified four key steps in the healthcare provider's workflow for conducting SICs with older adults in the ED. 
In the subsequent semi-structured interviews, we engaged with a broader group of healthcare providers members to gain a deeper understanding of the specific challenges and needs they encounter at each step of this workflow, as well as their perspectives on how AI tools might support their practices.


\subsection{Study Participants}
The participants in this study were healthcare providers who practice in the ED and have experience conducting SICs with older adults. While they do not specialize in or conduct research on serious illness communication, they routinely engage in these conversations as part of their clinical responsibilities. Their work environment is high-pressure and fast-paced, often involving complex cases and rotating day and night shifts, which makes their availability limited. 
To capture a holistic understanding of the interprofessional workflow and communication dynamics involved in SICs, we intentionally recruited nine U.S.-based healthcare providers across diverse roles, including two nurses and seven physicians.
Participants were identified through the professional networks of our expert interviewees and recruited using snowball sampling—a commonly used method for accessing highly specialized clinical populations.
Table~\ref{tab:demographics2} shows our participant demographics, department, roles, and years of practice.
%Our study was reviewed and approved by the first author's institution's Institutional Review Board, and the study complied with the approved procedure for ethical research practices of human subject protection.

\begin{table*}
  \caption{Demographics of the Subsequent Semi-Structured Interviews}
  \label{tab:demographics2}
  \begin{tabular}{cclcc} 
    \toprule
    P\# & Gender & Department & Job Title & Year of Practice \\ 
    \midrule
    P1 & Male & Emergency Department & Emergency Medicine Physician and Toxicologist & 30 years \\ 
    P2 & Female & Emergency Department & Nurse & 42 years \\
    P3 & Male & Emergency Department & Emergency Medicine Physician & 10 years \\ 
    P4 & Female & Emergency Department & Emergency Medicine Physician & 4 years \\
    P5 & Male & Emergency Department & Emergency Medicine Physician & 7 years \\ 
    P6 & Female & Emergency Department & Nurse & 20 years \\
    P7 & Male & Emergency Department & Emergency Medicine Physician and Intensivist & 20 years \\ 
    P8 & Male & Emergency Department & Emergency Medicine and Palliative Care Physician & 5 years \\
    P9 & Male & Emergency Department & Emergency and Critical Care Medicine Physician & 5 years \\
    \bottomrule
  \end{tabular}
\end{table*}

\subsection{Study Procedure}
We conducted semi-structured interviews remotely via Microsoft Teams, each lasting approximately 30 minutes.
Participants first described a recent experience conducting an SIC with an older adult in the ED. 
They then detailed specific challenges and needs experienced during each phase of their workflow (identification, preparation, conduction, and documentation).
Next, participants shared the existing frameworks and technologies they currently rely upon to support their SIC processes. 
Finally, we explored participants' perspectives regarding potential roles for AI tools.

To support participants in reflecting on AI opportunities, we used insights from earlier expert interviews to create illustrative examples of text-based AI support.
These were not part of the interview protocol per se, but were used only if participants struggled to articulate scenarios on their own.
Our intention was not to test these scenarios or restrict the conversation but rather to use them as reflective scaffolds—cognitive prompts that could help participants generate or refine their own ideas. 
Participants were encouraged to respond freely, expanding upon, critiquing, reframing, or entirely redefining the scenarios provided.
This approach reflects early-stage, exploratory design research practices where speculative but grounded examples can support participants’ imagination while preserving openness and participant agency.
The interviews were audio-recorded and transcribed with the participants' consent. 



After the interviews, we analyzed transcripts using both inductive and deductive thematic analysis methods~\cite{fereday2006demonstrating}. 
Two researchers from our team independently employed the inductive thematic analysis approach to analyze two transcripts and identified meaningful quotes and categorized these quotes into codes. 
Then, they resolved discrepancies among the codes and came up with key themes.
After the discussion, they used deductive thematic analysis to group similar codes and leveraged inductive thematic analysis to identify new codes.
They then discussed again and reached a consensus about the codes.
Finally, they grouped the codes into themes in each step of the SIC workflow.
To transparently report our findings, we indicate the prevalence of codes and themes across participants using the following terminology: "a few" refers to up to 20\% of participants, "some" indicates 21-50\%, "most" represents 51-80\%, and "nearly all" denotes 80\% or more of participants.







\section{Findings}
\label{sec:finding}
In this section, we presented the challenges and needs that clinical care teams face in their workflow of conducting SICs with older adult patients in the ED to address RQ1 in Sections \ref{sec:gaps} through \ref{sec:handoff}. 
Then we discussed AI opportunities about supporting clinical care teams in the workflow to address RQ2 in Section \ref{sec:ai}.

\subsection{Gaps in Real-Time Alignment Between Communication Needs and EHR}
\label{sec:gaps}
When older adult patients with serious illness arrive at the ED, nurses start a triage to evaluate patient health conditions.
During triage, nurses attempt to gather the patient's health history and understand the reason for the ED visit. 
However, P2 noted that not all patients provide the necessary details to support accurate assessment of their condition in their emergency situation. 
For instance, P2 described a patient who reported being in good health, but upon reviewing the EHR, she discovered the patient had stage IV cancer:
\begin{quote}
    \textit{``Maybe something doesn't seem quite right...from what you're telling me, it sounds like they're in pretty good health, but I'm looking at this patient and saying this patient is not in good health, so what's missing?''} (P2)
\end{quote}

While some patients are able to communicate with clinical care teams, others present significant communication barriers that complicate information gathering. 
Some patients may arrive at the ED in a coma or otherwise incapacitated, which makes them unable to communicate their medical history or current condition, or care preference to the clinical care team. 
When patients lack the capacity to communicate, clinical care teams typically turn to patients' families or surrogates (people who make medical decisions on behalf of a patient) to obtain the patient's essential information. 
However, some patients arrive at the ED alone, without family members or surrogates present. 
This situation makes it difficult for clinical care teams to fully understand the patient's health conditions or conduct a SIC to ascertain the patient’s care preferences. 
Thus, P1 noted that when the patients are unable to communicate and no surrogate is available, urgent clinical decision-making in the ED becomes significantly more complicated.
\begin{quote}
    \textit{``And oftentimes you get older individuals who don't have family members, or they can't be identified, and it makes the treatment sometimes trickier because they can't tell the story.''} (P1)
\end{quote}





\subsection{Clinical Care Teams Have Difficulties Accessing and Utilizing the EHR Data Prior to SICs in the ED}
\label{sec:ehr_data}
Many participants (P1, P4, P5, P7, P8, P9) noted that when patients present with life-threatening clinical indicators, such as intracranial hemorrhage, newly diagnosed malignancy, or frequent ED revisits, they recognized that the patients were at elevated risk of mortality.
If patients have a high risk of mortality, it normally means they need to receive aggressive treatment to save their lives. 
Before proceeding with such interventions, clinical care teams would check the EHR to find whether patients had SICs previously, and to access the documentation to understand patients’ treatment preferences, including DNI (i.e., do Not Intubate) and DNR (i.e., do Not Resuscitate).
These records are essential for aligning the urgent treatment in the ED with patient care preferences.
\begin{quote}
    \textit{``We're worried that we may hit a point very quickly, if not immediately where we are considering doing some kind of invasive procedure that they may or may not want.''} (P8)
\end{quote}

However, accessing reliable information about patient preferences presents several challenges.
Firstly, as P8 noted, the relevant details are often buried within lengthy progress notes that can cover the patient’s entire illness trajectory, which makes them difficult to locate and not clearly highlighted in the EHR system.
\begin{quote}
    \textit{``Talking about code status (DNI and DNR) is one small piece of that [SIC], but that can actually be shockingly hard to find in most EHRs or EMRs...it's usually not flagged in an obvious way... So it's like mentioned in a progress note, but there might be thousands of progress notes.''} (P8)
\end{quote}
 Even when clinical care teams locate relevant documentation in the EHR system, a few participants (P3, P7) reported that patients' goals of care and treatment preferences may have changed over time without corresponding updates to their records.  
 In other circumstances, some participants (P1, P4, P7, P8) encountered limited information availability altogether. 
 For example, when P7 searched for specific care preference keywords, the EHR returned only "not addressed," providing insufficient information to support clinical decision-making. 
Thus, a few participants (P3, P7) emphasized that having access to accurate and up-to-date patient information would be highly beneficial, as such information helps clinical care teams improve patient condition assessment and supports decisions about whether SICs are needed.

\begin{quote}
    \textit{``The information documented in the chart may not be accurate, the goals of care may have changed, and haven't been updated. Sometimes there's conflicting notes, and understanding what's right and current can be helpful.''} (P3)
\end{quote}






\subsection{Contextual Logistical and Emotional Constraints Undermining Preparation for Values-Based Emergency Care}
\label{sec:preparation}

Once clinical care teams identify the need for a SIC, they must prepare for it, yet they face a series of interconnected logistical and emotional constraints. 
Some participants (P4, P7, P8, P9) described difficulty finding the right moment to conduct SICs due to the high volume of patients and the fast-paced nature of the ED. 
Under time pressure,, clinical care teams need to be more selective about which patients receive SICs, as P7 noted. 
In addition to time constraints, the sensitive nature of SICs often leaves patients and families unprepared, which leads some participants (P3, P4, P6, P8, P9) to stress the need for quiet, private spaces. 
However, such spaces are often unavailable due to overcrowded ED conditions. P8 explained that some patients are placed in hallways amid noise and chaos while others remain in waiting rooms for 10 to 15 hours.

\begin{quote}
\textit{``I think in the emergency setting, it is usually [challenging] like physical, like [finding] time and space [to conduct the SIC]. So like I said, you know, even finding private care space sometimes is challenging. Having the time to have these conversations is really challenging.''} (P4)
\end{quote}

%Only P9 reported that finding private space was not challenging, as he typically conducts SIC at the patient's bedside. His challenge instead involved finding time to catch up on tasks delayed by SIC conversations, such as providing care for other patients. 

When time and space are secured, some participants (P1, P3, P4) noted that they often try to identify who else patients would like present during the conversation.  
If key family members or surrogate decision-makers are not physically present, clinical care teams often call them to ensure everyone remains informed. 
However, surrogates and caregivers are not always reachable. 
In cases where patients cannot communicate and no documented care preferences exist, clinical care teams typically default to aggressive treatment to preserve life.

%\begin{quote}
%\textit{``I'd like to talk to them about their condition and sort of their healthcare and if they'd like anyone else present for that conversation and if they want to invite anyone else.''} (P3)
%\end{quote}

Beyond logistics, preparing mentally and emotionally for SICs was described as more challenging. 
Many participants (P1, P2, P4, P5, P6, P9)shared that these conversations are emotionally demanding, particularly for those with less experience. 
A few participants (P4, P6) noted that SICs sometimes occur spontaneously without advance preparation time. 
P9 described the need to create an “emotional container” to help patients and families manage distress during difficult discussions. 
However, such emotional readiness is difficult to achieve, and P6 observed that many colleagues avoid initiating SICs because they feel unprepared.

\begin{quote}
\textit{``The emotional piece is much more complex, and it's why this issue has such great difficulty within dissemination and adoption.''} (P5)
\end{quote}

To support this emotional preparation, some participants mentioned training modules (P1, P6) and real-life practice (P1, P2, P7) as helpful. 
Moreover, personal experience significantly affects clinicians' perceived difficulty in conducting SICs mentally. 
P1 described how his experience providing long-term care for his parents helps him relate to patients and their family members during difficult times. Conversely, P5 described how losing his father to cancer made SICs more emotionally taxing, especially when caring for older adult cancer patients.

\begin{quote}
\textit{``That next year or two, I was emotionally different than I was before. These conversations were more emotional for me. I was more connected to the conversation as I just lost my father. Even I might tear up during these conversations when historically throughout my career, I never would cry or show emotion like that... You know how this hits home, you know, a clinician who lost a parent to cancer to go talk to a cancer patient at end of life might be extremely difficult, but maybe for someone else [it] might not be difficult.''} (P5)
\end{quote}





\subsection{Supporting Patient Sense-Making and Emotional Engagement During SICs Conduction}
\label{sec:conduction}
When clinical care teams prepare for conducting SICs with older adult patients in the ED, they encounter three key challenges: communicating undesirable and unexpected health conditions, building connection and trust within compressed timeframes, and making treatment decisions when patients cannot participate.
Delivering difficult diagnoses presents significant communication challenges. Some participants (P3, P4, P7, P8) found it particularly hard to communicate devastating health conditions (e.g., cancer diagnoses) to older adult patients and their families, especially when patients or families hold expectations that do not match clinical realities. 
Some families expect full recovery despite the severity of illness. This gap often leads to shock and distress, making the conversation more difficult. 
To address this challenge, a few participants noted that providing additional contextual information (P2, P9) and calibrating communication approaches based on patient understanding (P2) support acceptance of the information.
\begin{quote}
\textit{``I think it's often challenging when the goals of care don't necessarily align with reality. And there's an expectation that the patient's gonna recover from a condition that's essentially not recoverable. Or the expectations of the family or that there's going to be some type of sort of miraculous cure when that's not going to happen, that can be challenging.''} (P3)
\end{quote}

Beyond information delivery, some participants (P2, P5, P6, P9) emphasized the importance of building personal connections with patients. 
P2 described how she builds connections by finding common topics to initiate conversations, such as discussing patients' favorite sports teams or their children. 
Therefore, they can make the patient feel seen as a person, not just as a case to build trust. 
\begin{quote}
\textit{``Because if you don't make a connection, then your nursing is not personal to them (the patients). And then you feel like you're not treating their them personally, you're just treating cancer or you're just treating a heart attack.''} (P2)
\end{quote}

However, some participants (P2, P5, P8) noted that building a connection and establishing trust in the ED presents unique challenges. 
P5 explained that, unlike other care settings where providers may have long-standing relationships with patients, clinical care teams often meet patients for the first time in urgent, high-stress ED settings. 
As P5 described, this lack of history makes it harder to earn a patient’s trust in a short period of time.
\begin{quote}
\textit{``We're at a significant disadvantage in the emergency department as I am not their primary care doctor. I have not cared for them for a decade, you know, and earned all their trust and faith. They are meeting me at point blank, you know, and they have to develop faith and trust.''} (P5)
\end{quote}

%To compensate for these constraints, care teams employ various rapid rapport-building strategies, such as asking personal questions about where patients live or involving family members in conversations when appropriate, as P6 noted.
The third challenge occurs when older adult patients cannot participate conversationally due to conditions such as unconsciousness or breathing difficulties. 
Most participants (P1, P2, P4, P5, P7, P8, P9) identified this as a particularly complex situation. 
While P5 and P9 noted that patients are always the preferred participants for SICs, when patients cannot engage, clinical care teams must quickly identify alternative decision-makers, such as surrogates or family members, to conduct SICs and support clinical decision-making. 
However, this process becomes complicated when patients arrive without any family members, as P1 noted, potentially hindering SICs' conduct and delaying critical treatment decisions.
%multiple family members have varying levels of decision-making authority, as P4 described. The situation becomes even more challenging when
\begin{quote}
\textit{``you get older individuals who don't have family members, or they can't be identified, and it makes the treatment sometimes trickier because they can't tell the story.''} (P1)
\end{quote}





\subsection{Inadequate Handoff of Patient Values and Goals from Emergency Clinicians to Primary Teams}
\label{sec:handoff}

Following the completion of SICs, all participants indicated that they document summaries of SICs within the EHR system.
However, they reported challenges during the documentation process.
Participants (P5, P8) described the documentation as a time-consuming and burdensome process, especially in the ED. 
The high workload in the ED leaves clinical care teams with limited or no time for documentation during their scheduled shifts. 
As a result, some clinical care team members may be unable to document SICs promptly, while others must stay late or use unpaid personal time to complete this essential task.
P8 added that no effective method exists for documenting SICs during active shifts. 
\begin{quote}
\textit{``A lot of what you do is looking through a ton of data, trying to synthesize it, seeing the patient, addressing too many things in too little time, and then trying to document it and then do it, you know, 30 or 40 more times in a shift. And so many of us end up staying late or working unpaid hours, finishing charts because we care, and the system takes advantage of us.''} (P8)
\end{quote}

Once documented, the information serves two interconnected purposes: communicating with patients’ ongoing care teams to support clinical decision-making (P1, P4) and supporting the continuity of SICs across future encounters (P8, P9). 
However, there are obstacles to achieving these two purposes.
Communicating with patients’ ongoing care teams is challenging due to the complexity of care provider networks within EHR systems.
P1 described that EHRs list multiple clinical care team members (e.g., attending physicians, residents, nurse practitioners, and physician assistants) without clear indicators of who is currently responsible for care.
Even when clinical care teams identify the right person to connect, timing mismatches often prevent connection, particularly when ED teams work night shifts while other providers remain unavailable.
\begin{quote}
\textit{``You'll open up a patient's chart and there'll be so many healthcare providers, physicians, nurse practitioners, physician assistants, residents...You don't know who to call, and if you do, they're often not on calls.''} (P1)
\end{quote}

%The second critical function of documentation involves enabling care continuity, as a few participants (P8, P9) noted that documentation allows subsequent providers to continue SIC processes. 
%P5 emphasized that SICs represent an ongoing, evolving conversation rather than a singular ED event, making it essential to document SICs' progress and ensure accessibility for other care providers. 
Supporting the continuity of SICs is compromised by inconsistent documentation practices. 
P9 observed that clinical care teams document SICs content in various EHR locations: some create separate ED progress notes, others include information in ED final notes, and some use advance care planning (ACP) notes. 
This variability creates accessibility problems, as documentation not entered as ACP notes is unlikely to be revisited or seen by future clinical care teams, which potentially hinders other clinical care teams' ability to access the documentation and effectively follow up on SICs.
\begin{quote}
\textit{``I've seen variability where I've seen some people document it as a separate ED progress note. I've seen some people document as an ACP note. And then I've also seen some people just document it as part of the ED course that then populates into the final ED provider note.''} (P9)
\end{quote}






\subsection{Integrating AI into the SIC workflow in the ED}
\label{sec:ai}
\subsubsection{Opportunities for Integrating AI into the SIC workflow in the ED}
\label{sec:opportunities_for_ai}




When asked about the potential role of AI in their workflow, participants expressed strong interest in three areas that directly reflect earlier challenges: pre-conversation information synthesis for identification and preparation, real-time conversation support for conducting SICs, and post-conversation documentation assistance.
Building on the EHR access challenges identified in Section \ref{sec:ehr_data}, some participants (P3, P4, P7, P8) suggested that AI could extract and summarize key information, such as previous SICs, from extensive health records, which helps clinical care teams quickly understand patient health conditions and their care preference.
Moreover, AI could help identify individuals who else should be involved in SICs for a better preparation. 
%Some participants (P3, P4, P7, P8) specifically expressed the need for rapid access to previous SIC summaries, as these conversations often build upon earlier discussions but remain scattered across different EHR locations. 
\begin{quote}
\textit{``Anyone who's previously documented, like if there was a goal of care button, I could click and it would go through everything that's been documented on a patient's chart. Because maybe they had a conversation with a social worker a few weeks ago or their primary care doctor, and I just don't have the time to click through every note.''} (P4)
\end{quote}

Besides, participants described opportunities for AI to support conversations as they unfold. 
Some (P4, P5, P6) imagined real-time systems that could listen passively, when consent is given, and offer contextually relevant question suggestions.
P6 explained that this AI feature could be especially helpful for clinical care teams with less experience conducting SICs. 
He suggested that AI could recommend contextually appropriate follow-up questions based on ongoing conversation content, which helps to sustain meaningful dialogue and more effectively elicit patient care preferences and goals of care. 
This real-time support addresses the communication challenges identified in Section \ref{sec:conduction}.%, where clinical care teams struggle to navigate sensitive topics while building trust under time pressure.



Beyond guiding individual conversations, P5 emphasized the value AI in helping to track what parts of the SIC had been completed.
He noted that SICs conducted in the ED represent merely the initial step in ongoing dialogues that continue throughout a patient's illness journey. 
Since comprehensive SICs can extend to an hour, but ED time constraints severely limit coverage of all necessary topics, a few participants (P8, P9) mentioned that ED-focused conversations must prioritize short-term goals. 
One of the important short-term goals is determining patient preferences for aggressive treatment to support immediate clinical decision-making. 
Because of these time constraints, P5 emphasized that AI could ambient listen to conversations and record progress, enabling subsequent care providers to understand which topics were addressed and which require attention in future encounters.
\begin{quote}
\textit{``And you know, you guys (researcher) define what those six things [that needed to be gotten done in SICs] are. I can only maybe accomplish one or two of them [in the ED]. The AI recognizes it and is able to inform the next provider. 'Hey, [the previous care provider] was only able to get through one and two, you know, consider focusing on three, four, and five'.''} (P5)
\end{quote}


Finally, many participants (P1, P3, P4, P5, P7, P8) expressed strong interest in AI-generated SIC summaries to addressing the substantial documentation burden identified in Section \ref{sec:handoff}.
Because SICs can be lengthy and emotionally complex, clinical care teams must distill large amounts of SICs into concise, clinically useful records. 
P3 suggested that AI could filter out unrelated conversation details and highlight patient goals and care preferences. 
Although many participants prefer AI summarization, others prefer different ways for AI to support documentation. 
For example, P9 prefers viewing the full conversation text with key information highlighted, while P1 proposes that AI systems could offer structured templates or word prompts to guide note creation. 
Regardless of how AI is used to support documentation, P8 estimated that automating 80\% of documentation work with AI could cut post-shift charting time in half, freeing up time for direct patient care.
\begin{quote}
\textit{``But if AI could offload even say 80 percent of that (documentation) and then the other 20 percent you're tweaking and verifying the transcript or, you know, the output, that would save close to half of my working hours that I could actually be spending with seeing more patients.''} (P8)
\end{quote}







\subsubsection{Concerns About Integrating AI into the SIC workflow in the ED}
\label{sec:concerns_about_ai}

While participants expressed enthusiasm for AI support opportunities, they also articulated important concerns about integrating AI into SICS.
Their worries focused on preserving human connection, ensuring trustworthiness, and maintaining clinical accuracy.
Some participants (P1, P3, P5, P6, P9) frequently noted the potential risk that AI might diminish the deeply human aspect of SICs. 
%The communication between clinical care teams and patients represents more than a structured information exchange—it constitutes "a human moment" (P5) that is "deeply personal" (P3). 
Clinician-patient interactions during these conversations represent more than structured information exchanges—they are highly personal moments characterized by emotional depth.
Participants worried that introducing AI could lead clinicians to rely excessively on technology-driven prompts, potentially reducing the genuine emotional engagement that patients value.
For instance, P3 was concerned that patients could perceive conversations assisted by AI as mechanical rather than sincere, thus undermining the quality of the interaction.

\begin{quote}
\textit{``if there's a perception that the physician is just using an electronic tool to ask [the] right questions, that's not really sort of coming from the heart, that could be negatively perceived.''} (P3)
\end{quote}

Moreover, some participants (P1, P4, P5, P6, P9) worried that AI integration might create distracting and disrespectful interactions when clinical care teams attempt to build connections with patients. 
They emphasized that well-conducted conversations require clinicians' undivided attention and direct eye contact. 
Frequent or noticeable interaction with computer screens could diminish the clinician’s presence, which potentially disrespects the gravity and intimacy of these sensitive discussions.
P6 specifically underscored the importance of face-to-face conversations without computer screen barriers.

\begin{quote}
\textit{``And I just think these conversations are like worthy of someone sitting down with you face to face, not having a computer screen in front of them.''} (P6)
\end{quote}

Trust and credibility of AI tools emerged as another critical concern. 
Some participants (P1, P5, P7) emphasized the necessity of thorough data validation before integrating AI into their workflows.
Specifically, P1 noted that personal adoption of AI would heavily depend on endorsements by trusted colleagues and credible evidence supporting AI's clinical validity. 
In addition to ensuring trust between clinical care teams and AI tools, participants emphasized that protecting patient privacy by obtaining explicit patient consent and providing clear opt-out options for AI use during SICs is essential to maintain patient trust in clinical care teams.
%This concern reflects the high stakes of SICs, where trust between clinical care teams and patients forms the foundation for meaningful dialogue about values, goals, and care preferences.



Finally, some participants (P3, P4, P7, P9) expressed significant concerns about the accuracy and clinical relevance of AI summarization for documentation. 
They worried that AI might overemphasize irrelevant content while failing to adequately highlight the information most relevant to clinical care teams. 
%P4 and P9 noted that AI-identified important content might not align with what clinical care teams consider most clinically relevant, potentially leading to inappropriate clinical responses. 
P4 provided an example of how AI might mistakenly elevate minor patient comments, such as a casual mention of "chest pain", to clinically significant events, which potentially leads to unnecessary medical interventions and resource usage. 
Such errors could result from the lack of clinical context or nuanced interpretation, further highlighting the importance of human oversight.
Thus, some participants (P3, P7, P9) emphasized the critical importance of clinician review and verification processes before finalizing any AI-generated summaries, ensuring that automated assistance enhances rather than compromises clinical decision-making.

\begin{quote}
\textit{``Although the final sign off is going to be clinician reviewing the summary of what AI note taking would be, right? ... We still have to read it again, make sure that's actually all accurate.''} (P7)
\end{quote}
